Fine-Grained Semantic Segmentation of Motion Capture Data using Dilated Temporal Fully-Convolutional Networks

Human motion capture data has been widely used in data-driven character animation. In order to generate realistic, natural-looking motions, most data-driven approaches require considerable efforts of pre-processing, including motion segmentation and annotation. Existing (semi-) automatic solutions either require hand-crafted features for motion segmentation or do not produce the semantic annotations required for motion synthesis and building large-scale motion databases. In addition, human labeled annotation data suffers from inter- and intra-labeler inconsistencies by design. We propose a semi-automatic framework for semantic segmentation of motion capture data based on supervised machine learning techniques. It first transforms a motion capture sequence into a ``motion image'' and applies a convolutional neural network for image segmentation. Dilated temporal convolutions enable the extraction of temporal information from a large receptive field. Our model outperforms two state-of-the-art models for action segmentation, as well as a popular network for sequence modeling. Most of all, our method is very robust under noisy and inaccurate training labels and thus can handle human errors during the labeling process.

==> EGauthorGuidelines-body-sub.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.02, Jan 25, 2017


\title[EG \LaTeX\ Author Guidelines]%
      {\LaTeX\ Author Guidelines for EUROGRAPHICS Proceedings Manuscripts}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
%\author[D. Fellner \& S. Behnke]
\author[SUBMISSION ID]{SUBMISSION ID}
% {\parbox{\textwidth}{\centering D.\,W. Fellner\thanks{Chairman Eurographics Publications Board}$^{1,2}$\orcid{0000-0001-7756-0901}
%         and S. Behnke$^{2}$\orcid{0000-0001-5923-423X} 
% %        S. Spencer$^2$\thanks{Chairman Siggraph Publications Board}
%         }
%         \\
% % For Computer Graphics Forum: Please use the abbreviation of your first name.
% {\parbox{\textwidth}{\centering $^1$TU Darmstadt \& Fraunhofer IGD, Germany\\
%          $^2$Graz University of Technology, Institute of Computer Graphics and Knowledge Visualization, Austria
% %        $^2$ Another Department to illustrate the use in papers from authors
% %             with different affiliations
%        }
% }
%}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

% uncomment for using teaser
% \teaser{
%  \includegraphics[width=\linewidth]{eg_new}
%  \centering
%   \caption{New EG Logo}
% \label{fig:teaser}
%}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract}
   The ABSTRACT is to be in fully-justified italicized text, 
   between two horizontal lines,
   in one-column format, 
   below the author and affiliation information. 
   Use the word ``Abstract'' as the title, in 9-point Times, boldface type, 
   left-aligned to the text, initially capitalized. 
   The abstract is to be in 9-point, single-spaced type.
   The abstract may be up to 3 inches (7.62 cm) long. \\
   Leave one blank line after the abstract, 
   then add the subject categories according to the ACM Classification Index 
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see http://www.acm.org/about/class/1998)
% \begin{classification} % according to http:http://www.acm.org/about/class/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
   (see http://www.acm.org/about/class/class/2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010352.10010381</concept_id>
<concept_desc>Computing methodologies~Collision detection</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010588.10010559</concept_id>
<concept_desc>Hardware~Sensors and actuators</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010584.10010587</concept_id>
<concept_desc>Hardware~PCB design and layout</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[300]{Computing methodologies~Collision detection}
\ccsdesc[300]{Hardware~Sensors and actuators}
\ccsdesc[100]{Hardware~PCB design and layout}


\printccsdesc   
\end{abstract}  
%-------------------------------------------------------------------------
\section{Introduction}

Please follow the steps outlined in this document very carefully when
submitting your manuscript to Eurographics.

You may as well use the \LaTeX\ source as a template to typeset your own
paper. In this case we encourage you to also read the \LaTeX\ comments
embedded in the document.

%-------------------------------------------------------------------------
\section{Instructions}

Please read the following carefully.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts,
must be kept within a print area %6.31 inches (16.03 cm) 
7 inches (17.7 cm) wide by
%9.10 inches (23.13 cm) 
9.44 inches (24 cm) high. Do not write or print anything
outside the print area. Number your pages on odd sites right
above, on even sites left above, no page number on the first site.
Do not use page numbering within the final version of your paper.


%------------------------------------------------------------------------
\subsection{Formatting your paper}

% All text with the exception of the abstract must be in a two-column format.
% The total allowable width of the text area -- including header and footer
% lines -- is 161\,mm (6.34 inch) wide by 231\,mm (9.10 inch) high.
% 
% Columns are to be 76\,mm (3.0 inch) wide, with a 8\,mm (0.315 inch) space 
% between them.

All text with the exception of the abstract must be in a two-column format.
The total allowable width of the text area -- including header and footer
lines -- is 177\,mm (7 inch) wide by 245\,mm (9.64 inch) high.

Columns are to be 84\,mm (3.3 inch) wide, with a 8\,mm (0.315 inch) space 
between them.

The space between the header line and the first line of the text body and
between the last line of the text body and the footer line is 5\,mm
(0.196 inch) each.

%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If
neither is available on your word processor, please use the font
closest in appearance to Times that you have access to. Only
Type-1 fonts will be accepted.

MAIN TITLE. The title should be in Times 17-point, boldface type and
centered. Capitalize the first letter of nouns, pronouns, verbs, adjectives,
and adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title and
printed in Times 9-point, non-boldface type. This information is to be
followed by two blank lines.

The ABSTRACT ist to be in a one-column format. The MAIN TEXT is to be in a
two-column format.

MAIN TEXT. Type main text in 9-point Times, single-spaced. Do \emph{not} use
double-spacing. All paragraphs should be indented 1 em (the length of the
dash in the actual font). Make sure your text is fully justified -- that is,
flush left and flush right. Please do not place any additional blank lines
between paragraphs. Figure and table captions should be 9-point Times
boldface type as in Figure~\ref{fig:firstExample}.

\noindent Long captions should be set as in Figure~\ref{fig:ex1} or
Figure~\ref{fig:ex3}.

\begin{figure}[htb]
   % an empty figure just consisting of the caption lines
   \caption{\label{fig:ex1}
     'Empty' figure only to serve as an example of long caption requiring 
     more than one line. It is not typed centered but aligned on both sides.}
\end{figure}

\noindent
Figures which need the full textwidth can be typeset as Figure~\ref{fig:ex3}.

\noindent Callouts should be 9-point Times, non-boldface type. Initially
capitalize only the first word of section titles and first-, second-, and
third-order headings.

FIRST-ORDER HEADINGS. (For example, \textbf{1. Introduction}) should be Times
9-point boldface, initially capitalized, flush left, with one blank line
before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, \textbf{2.1. Language}) should be Times
9-point boldface, initially capitalized, flush left, with one blank line
before, and one after. If you require a third-order heading (we discourage
it), use 9-point Times, boldface, initially capitalized, flush left, preceded
by one blank line, followed by a period and your text on the same line.

The headline \emph{(authors / title)} must be shortened if it uses the full 
two column width of the main text.
There must be enough space for the page numbers. Please use ``et al.'' if 
there are more than three authors and specify a shortened version for your title.
%-------------------------------------------------------------------------
\subsection{Footnotes}

Please do \emph{not} use footnotes at all!


%-------------------------------------------------------------------------
\subsection{References}

List all bibliographical references in 9-point Times, single-spaced, at the
end of your paper in alphabetical order. When referenced in the text, enclose
the citation index in square brackets, for example~\cite{Lous90}. Where
appropriate, include the name(s) of editors of referenced books.

For your references please use the following algorithm:
\begin{itemize} 
\item \textbf{one} author: first 3 chars plus year -- 
      e.g.\ \cite{Lous90}
\item \textbf{two}, \textbf{three} or \textbf{four} authors: first char
      of each family name plus year --  e.g.\ \cite{Fellner-Helmberg93} 
      or \cite{Kobbelt97-USHDR} or \cite{Lafortune97-NARF}
\item \textbf{more than 4} authors: first char of family name from 
      first 3 authors followed by a '*' followed by the year -- 
      e.g.\ \cite{Buhmann:1998:DCQ} or \cite{FolDamFeiHug.etal93} 
\end{itemize}

For BibTeX users a style file \ \texttt{eg-alpha.bst} \ is available which
uses the above algorithm.

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.

%%%
%%% Figure 1
%%%
\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.8\linewidth]{sampleFig}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %
  \parbox[t]{.9\columnwidth}{\relax
           For all figures please keep in mind that you \textbf{must not}
           use images with transparent background! 
           }
  %
  \caption{\label{fig:firstExample}
           Here is a sample figure.}
\end{figure}

If your paper includes images, it is very important that they are of
sufficient resolution to be faithfully reproduced.

To determine the optimum size (width and height) of an image, measure
the image's size as it appears in your document (in millimeters), and
then multiply those two values by 12. The resulting values are the
optimum $x$ and $y$ resolution, in pixels, of the image. Image quality
will suffer if these guidelines are not followed.

Example 1: 
%
An image measures 50\,mm by 75\,mm when placed in a document. This
image should have a resolution of no less than 600 pixels by 900
pixels in order to be reproduced faithfully.

Example 2: 
%
Capturing a screenshot of your entire $1024 \times 768$ pixel display
monitor may be useful in illustrating a concept from your research. In
order to be reproduced faithfully, that $1024 \times 768$ image should
be no larger than 85 mm by 64 mm (approximately) when placed in your
document.


%-------------------------------------------------------------------------
\subsection{Color}

\textbf{Please observe:} as of 2003 publications in the proceedings of the
Eurographics Conference can use color images throughout the paper. No
separate color tables are necessary.

However, workshop proceedings might have different agreements! 
Figure~\ref{fig:ex3} is an example for creating color plates.

%------------------------------------------------------------------------
\subsection{Embedding of Hyperlinks / Typesetting of URLs}

Due to the use of the package \texttt{hyperref} the original behavior
of the command $\backslash$\texttt{url} from the package \texttt{url}
is not available. To circumvent this problem we either recommend to
use the command $\backslash$\texttt{httpAddr} from the 
included package \texttt{egweblnk} (see below) or to replace the
command $\backslash$\texttt{url} by the command $\backslash$\texttt{webLink} 
-- e.g. in cases where $\backslash$\texttt{url} has been used
widely in BibTeX-References. In the latter case we suggest to run
BibTeX as usual and then replace all occurences of $\backslash$\texttt{url}  by
$\backslash$\texttt{webLink}

\noindent
The provided commands for hyperlinks, in a nutshell, are:

\begin{description} \itemsep 1ex
\item [\webLinkFont $\backslash$httpAddr \{URL without leading 'http:'\}]
      \mbox{}\\
      e.g. \  \httpAddr{//diglib.eg.org/EG/DL/WS}

\item[\webLinkFont $\backslash$ftpAddr \{URL without leading 'ftp:'\}]
      \mbox{}\\
      e.g. \  \ftpAddr{//www.eg.org/EG/DL/ftpupload}

\item[\webLinkFont $\backslash$URL \{url\}]
      \mbox{}\\
      e.g. \  \URL{http://www.eg.org/EG/DL/WS}

\item[\webLinkFont $\backslash$MailTo \{Email addr\}]
      \mbox{}\\
      e.g. \  \MailTo{publishing@eg.org}

\item[\webLinkFont $\backslash$MailToNA \{emailName\}\{@emailSiteAddress\}]
      \mbox{}\\
      e.g. \  \MailToNA{publishing}{@eg.org}

\item[\webLinkFont $\backslash$webLink\{URL without hyperlink creation\}]
      \mbox{}\\
      e.g. \  \webLink{http://www.eg.org/some_arbitrary_long/but_useless/URL}

\end{description}


%------------------------------------------------------------------------
\subsection{PDF Generation}

Your final paper should be delivered as a PDF document with all typefaces
embedded. \LaTeX{} users should use \texttt{dvips} and \texttt{ps2pdf} to
create this PDF document. Adobe Acrobat Distiller may be used in place of
\texttt{ps2pdf}.

Adobe PDFWriter is \emph{not} acceptable for use. Documents created with
PDFWriter will be returned to the author for revision. \texttt{pdftex} and
\texttt{pdflatex} (and its variants) can be used only if the author can
make certain that all typefaces are embedded and images are not downsampled
or subsampled during the PDF creation process.

Users with no access to these PDF creation tools should make available a
PostScript file and we will make a PDF document from it.


The PDF file \emph{must not} be change protected.

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: dvips / ps2pdf / etc.}

\noindent
\texttt{dvips} should be invoked with the \texttt{-Ppdf} and \texttt{-G0}
flags in order to use Type 1 PostScript typefaces:

\begin{verbatim}
    dvips -t a4 -Ppdf -G0 -o my.ps my.dvi
\end{verbatim}


\noindent
If you are using version 7.x of GhostScript, please use the following method of invoking \texttt{ps2pdf}, in
order to embed all typefaces and ensure that images are not downsampled or subsampled in the PDF
creation process:

\begin{verbatim}
  ps2pdf -dMaxSubsetPct=100 \
         -dCompatibilityLevel=1.3 \
         -dSubsetFonts=true \
         -dEmbedAllFonts=true \
         -dAutoFilterColorImages=false \
         -dAutoFilterGrayImages=false \
         -dColorImageFilter=/FlateEncode \
         -dGrayImageFilter=/FlateEncode \
         -dMonoImageFilter=/FlateEncode \
         mypaper.ps mypaper.pdf
\end{verbatim}


If you are using version 8.x of GhostScript, please use this method in place of the example above:
\begin{verbatim}
  ps2pdf -dPDFSETTINGS=/prepress \
         -dCompatibilityLevel=1.3 \
         -dAutoFilterColorImages=false \
         -dAutoFilterGrayImages=false \
         -dColorImageFilter=/FlateEncode \
         -dGrayImageFilter=/FlateEncode \
         -dMonoImageFilter=/FlateEncode \
         -dDownsampleColorImages=false \
         -dDownsampleGrayImages=false \
         mypaper.ps mypaper.pdf
\end{verbatim}

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: pdftex / pdflatex / etc.}

\noindent
Configuration of these tools to embed all typefaces can be accomplished by editing the \texttt{updmap.cfg} file
to enable inclusion of the standard (or base) 14 typefaces.

Linux users can run the \texttt{updmap} script to do this:
\begin{verbatim}
updmap --setoption pdftexDownloadBase14 true
\end{verbatim}

Windows users should edit the \texttt{updmap.cfg} files found in their TeX installation directories (one or both
of the following may be present):
\begin{verbatim}
  INSTALLDIR\texmf\web2c\updmap.cfg
  INSTALLDIR\localtexmf\miktex\config\updmap.cfg
\end{verbatim}

Ensure the value for \texttt{pdftexDownloadBase14} is "true," and then follow the instructions found here:
\httpAddr{//docs.miktex.org/manual/} to update your MikTeX installation.

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: Acrobat Distiller}

We recommend to use a Distiller job options file that embeds
all typefaces and does not downsample or subsample images when creating the PDF document.
%------------------------------------------------------------------------
\subsection{Exclusive License Form}

You must include your signed Eurographics Exclusive License Form 
when you submit your finished paper. We MUST have this form before
your paper can be published in the proceedings.

%-------------------------------------------------------------------------
\subsection{Conclusions}

Please direct any questions to the production editor in charge of
these proceedings.

%-------------------------------------------------------------------------

%\bibliographystyle{eg-alpha}
\bibliographystyle{eg-alpha-doi}

\bibliography{egbibsample}

%-------------------------------------------------------------------------
\newpage


\begin{figure*}[tbp]
  \centering
  \mbox{} \hfill
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.3\linewidth]{sampleFig}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.3\linewidth, bb=39 696 126 756]{sampleFig}
  \hfill
  \includegraphics[width=.3\linewidth]{sampleFig}
  \hfill \mbox{}
  \caption{\label{fig:ex3}%
           For publications with color tables (i.e., publications not offering
           color throughout the paper) please \textbf{observe}: 
           for the printed version -- and ONLY for the printed
           version -- color figures have to be placed in the last page.
           \newline
           For the electronic version, which will be converted to PDF before
           making it available electronically, the color images should be
           embedded within the document. Optionally, other multimedia
           material may be attached to the electronic version. }
\end{figure*}

\end{document}


==> EGauthorGuidelines-body.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.02, Jan 25, 2017


\title[EG \LaTeX\ Author Guidelines]%
      {\LaTeX\ Author Guidelines for EUROGRAPHICS Proceedings Manuscripts}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[D. Fellner \& S. Behnke]
{\parbox{\textwidth}{\centering D.\,W. Fellner\thanks{Chairman Eurographics Publications Board}$^{1,2}$\orcid{0000-0001-7756-0901}
        and S. Behnke$^{2}$\orcid{0000-0001-5923-423X} 
%        S. Spencer$^2$\thanks{Chairman Siggraph Publications Board}
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$TU Darmstadt \& Fraunhofer IGD, Germany\\
         $^2$Graz University of Technology, Institute of Computer Graphics and Knowledge Visualization, Austria
%        $^2$ Another Department to illustrate the use in papers from authors
%             with different affiliations
       }
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

% uncomment for using teaser
% \teaser{
%  \includegraphics[width=\linewidth]{eg_new}
%  \centering
%   \caption{New EG Logo}
% \label{fig:teaser}
%}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract}
   The ABSTRACT is to be in fully-justified italicized text, 
   between two horizontal lines,
   in one-column format, 
   below the author and affiliation information. 
   Use the word ``Abstract'' as the title, in 9-point Times, boldface type, 
   left-aligned to the text, initially capitalized. 
   The abstract is to be in 9-point, single-spaced type.
   The abstract may be up to 3 inches (7.62 cm) long. \\
   Leave one blank line after the abstract, 
   then add the subject categories according to the ACM Classification Index 
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see http://www.acm.org/about/class/1998)
% \begin{classification} % according to http:http://www.acm.org/about/class/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
   (see http://www.acm.org/about/class/class/2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010352.10010381</concept_id>
<concept_desc>Computing methodologies~Collision detection</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010588.10010559</concept_id>
<concept_desc>Hardware~Sensors and actuators</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010584.10010587</concept_id>
<concept_desc>Hardware~PCB design and layout</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[300]{Computing methodologies~Collision detection}
\ccsdesc[300]{Hardware~Sensors and actuators}
\ccsdesc[100]{Hardware~PCB design and layout}


\printccsdesc   
\end{abstract}  
%-------------------------------------------------------------------------
\section{Introduction}

Please follow the steps outlined in this document very carefully when
submitting your manuscript to Eurographics.

You may as well use the \LaTeX\ source as a template to typeset your own
paper. In this case we encourage you to also read the \LaTeX\ comments
embedded in the document.

%-------------------------------------------------------------------------
\section{Instructions}

Please read the following carefully.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts,
must be kept within a print area %6.31 inches (16.03 cm) 
7 inches (17.7 cm) wide by
%9.10 inches (23.13 cm) 
9.44 inches (24 cm) high. Do not write or print anything
outside the print area. Number your pages on odd sites right
above, on even sites left above, no page number on the first site.
Do not use page numbering within the final version of your paper.


%------------------------------------------------------------------------
\subsection{Formatting your paper}

% All text with the exception of the abstract must be in a two-column format.
% The total allowable width of the text area -- including header and footer
% lines -- is 161\,mm (6.34 inch) wide by 231\,mm (9.10 inch) high.
% 
% Columns are to be 76\,mm (3.0 inch) wide, with a 8\,mm (0.315 inch) space 
% between them.

All text with the exception of the abstract must be in a two-column format.
The total allowable width of the text area -- including header and footer
lines -- is 177\,mm (7 inch) wide by 245\,mm (9.64 inch) high.

Columns are to be 84\,mm (3.3 inch) wide, with a 8\,mm (0.315 inch) space 
between them.

The space between the header line and the first line of the text body and
between the last line of the text body and the footer line is 5\,mm
(0.196 inch) each.

%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If
neither is available on your word processor, please use the font
closest in appearance to Times that you have access to. Only
Type-1 fonts will be accepted.

MAIN TITLE. The title should be in Times 17-point, boldface type and
centered. Capitalize the first letter of nouns, pronouns, verbs, adjectives,
and adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title and
printed in Times 9-point, non-boldface type. This information is to be
followed by two blank lines.

The ABSTRACT ist to be in a one-column format. The MAIN TEXT is to be in a
two-column format.

MAIN TEXT. Type main text in 9-point Times, single-spaced. Do \emph{not} use
double-spacing. All paragraphs should be indented 1 em (the length of the
dash in the actual font). Make sure your text is fully justified -- that is,
flush left and flush right. Please do not place any additional blank lines
between paragraphs. Figure and table captions should be 9-point Times
boldface type as in Figure~\ref{fig:firstExample}.

\noindent Long captions should be set as in Figure~\ref{fig:ex1} or
Figure~\ref{fig:ex3}.

\begin{figure}[htb]
   % an empty figure just consisting of the caption lines
   \caption{\label{fig:ex1}
     'Empty' figure only to serve as an example of long caption requiring 
     more than one line. It is not typed centered but aligned on both sides.}
\end{figure}

\noindent
Figures which need the full textwidth can be typeset as Figure~\ref{fig:ex3}.

\noindent Callouts should be 9-point Times, non-boldface type. Initially
capitalize only the first word of section titles and first-, second-, and
third-order headings.

FIRST-ORDER HEADINGS. (For example, \textbf{1. Introduction}) should be Times
9-point boldface, initially capitalized, flush left, with one blank line
before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, \textbf{2.1. Language}) should be Times
9-point boldface, initially capitalized, flush left, with one blank line
before, and one after. If you require a third-order heading (we discourage
it), use 9-point Times, boldface, initially capitalized, flush left, preceded
by one blank line, followed by a period and your text on the same line.

The headline \emph{(authors / title)} must be shortened if it uses the full 
two column width of the main text.
There must be enough space for the page numbers. Please use ``et al.'' if 
there are more than three authors and specify a shortened version for your title.
%-------------------------------------------------------------------------
\subsection{Footnotes}

Please do \emph{not} use footnotes at all!


%-------------------------------------------------------------------------
\subsection{References}

List all bibliographical references in 9-point Times, single-spaced, at the
end of your paper in alphabetical order. When referenced in the text, enclose
the citation index in square brackets, for example~\cite{Lous90}. Where
appropriate, include the name(s) of editors of referenced books.

For your references please use the following algorithm:
\begin{itemize} 
\item \textbf{one} author: first 3 chars plus year -- 
      e.g.\ \cite{Lous90}
\item \textbf{two}, \textbf{three} or \textbf{four} authors: first char
      of each family name plus year --  e.g.\ \cite{Fellner-Helmberg93} 
      or \cite{Kobbelt97-USHDR} or \cite{Lafortune97-NARF}
\item \textbf{more than 4} authors: first char of family name from 
      first 3 authors followed by a '*' followed by the year -- 
      e.g.\ \cite{Buhmann:1998:DCQ} or \cite{FolDamFeiHug.etal93} 
\end{itemize}

For BibTeX users a style file \ \texttt{eg-alpha.bst} \ is available which
uses the above algorithm.

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.

%%%
%%% Figure 1
%%%
\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.8\linewidth]{sampleFig}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %
  \parbox[t]{.9\columnwidth}{\relax
           For all figures please keep in mind that you \textbf{must not}
           use images with transparent background! 
           }
  %
  \caption{\label{fig:firstExample}
           Here is a sample figure.}
\end{figure}

If your paper includes images, it is very important that they are of
sufficient resolution to be faithfully reproduced.

To determine the optimum size (width and height) of an image, measure
the image's size as it appears in your document (in millimeters), and
then multiply those two values by 12. The resulting values are the
optimum $x$ and $y$ resolution, in pixels, of the image. Image quality
will suffer if these guidelines are not followed.

Example 1: 
%
An image measures 50\,mm by 75\,mm when placed in a document. This
image should have a resolution of no less than 600 pixels by 900
pixels in order to be reproduced faithfully.

Example 2: 
%
Capturing a screenshot of your entire $1024 \times 768$ pixel display
monitor may be useful in illustrating a concept from your research. In
order to be reproduced faithfully, that $1024 \times 768$ image should
be no larger than 85 mm by 64 mm (approximately) when placed in your
document.


%-------------------------------------------------------------------------
\subsection{Color}

\textbf{Please observe:} as of 2003 publications in the proceedings of the
Eurographics Conference can use color images throughout the paper. No
separate color tables are necessary.

However, workshop proceedings might have different agreements! 
Figure~\ref{fig:ex3} is an example for creating color plates.

%------------------------------------------------------------------------
\subsection{Embedding of Hyperlinks / Typesetting of URLs}

Due to the use of the package \texttt{hyperref} the original behavior
of the command $\backslash$\texttt{url} from the package \texttt{url}
is not available. To circumvent this problem we either recommend to
use the command $\backslash$\texttt{httpAddr} from the 
included package \texttt{egweblnk} (see below) or to replace the
command $\backslash$\texttt{url} by the command $\backslash$\texttt{webLink} 
-- e.g. in cases where $\backslash$\texttt{url} has been used
widely in BibTeX-References. In the latter case we suggest to run
BibTeX as usual and then replace all occurences of $\backslash$\texttt{url}  by
$\backslash$\texttt{webLink}

\noindent
The provided commands for hyperlinks, in a nutshell, are:

\begin{description} \itemsep 1ex
\item [\webLinkFont $\backslash$httpAddr \{URL without leading 'http:'\}]
      \mbox{}\\
      e.g. \  \httpAddr{//diglib.eg.org/EG/DL/WS}

\item[\webLinkFont $\backslash$ftpAddr \{URL without leading 'ftp:'\}]
      \mbox{}\\
      e.g. \  \ftpAddr{//www.eg.org/EG/DL/ftpupload}

\item[\webLinkFont $\backslash$URL \{url\}]
      \mbox{}\\
      e.g. \  \URL{http://www.eg.org/EG/DL/WS}

\item[\webLinkFont $\backslash$MailTo \{Email addr\}]
      \mbox{}\\
      e.g. \  \MailTo{publishing@eg.org}

\item[\webLinkFont $\backslash$MailToNA \{emailName\}\{@emailSiteAddress\}]
      \mbox{}\\
      e.g. \  \MailToNA{publishing}{@eg.org}

\item[\webLinkFont $\backslash$webLink\{URL without hyperlink creation\}]
      \mbox{}\\
      e.g. \  \webLink{http://www.eg.org/some_arbitrary_long/but_useless/URL}

\end{description}


%------------------------------------------------------------------------
\subsection{PDF Generation}

Your final paper should be delivered as a PDF document with all typefaces
embedded. \LaTeX{} users should use \texttt{dvips} and \texttt{ps2pdf} to
create this PDF document. Adobe Acrobat Distiller may be used in place of
\texttt{ps2pdf}.

Adobe PDFWriter is \emph{not} acceptable for use. Documents created with
PDFWriter will be returned to the author for revision. \texttt{pdftex} and
\texttt{pdflatex} (and its variants) can be used only if the author can
make certain that all typefaces are embedded and images are not downsampled
or subsampled during the PDF creation process.

Users with no access to these PDF creation tools should make available a
PostScript file and we will make a PDF document from it.


The PDF file \emph{must not} be change protected.

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: dvips / ps2pdf / etc.}

\noindent
\texttt{dvips} should be invoked with the \texttt{-Ppdf} and \texttt{-G0}
flags in order to use Type 1 PostScript typefaces:

\begin{verbatim}
    dvips -t a4 -Ppdf -G0 -o my.ps my.dvi
\end{verbatim}


\noindent
If you are using version 7.x of GhostScript, please use the following method of invoking \texttt{ps2pdf}, in
order to embed all typefaces and ensure that images are not downsampled or subsampled in the PDF
creation process:

\begin{verbatim}
  ps2pdf -dMaxSubsetPct=100 \
         -dCompatibilityLevel=1.3 \
         -dSubsetFonts=true \
         -dEmbedAllFonts=true \
         -dAutoFilterColorImages=false \
         -dAutoFilterGrayImages=false \
         -dColorImageFilter=/FlateEncode \
         -dGrayImageFilter=/FlateEncode \
         -dMonoImageFilter=/FlateEncode \
         mypaper.ps mypaper.pdf
\end{verbatim}


If you are using version 8.x of GhostScript, please use this method in place of the example above:
\begin{verbatim}
  ps2pdf -dPDFSETTINGS=/prepress \
         -dCompatibilityLevel=1.3 \
         -dAutoFilterColorImages=false \
         -dAutoFilterGrayImages=false \
         -dColorImageFilter=/FlateEncode \
         -dGrayImageFilter=/FlateEncode \
         -dMonoImageFilter=/FlateEncode \
         -dDownsampleColorImages=false \
         -dDownsampleGrayImages=false \
         mypaper.ps mypaper.pdf
\end{verbatim}

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: pdftex / pdflatex / etc.}

\noindent
Configuration of these tools to embed all typefaces can be accomplished by editing the \texttt{updmap.cfg} file
to enable inclusion of the standard (or base) 14 typefaces.

Linux users can run the \texttt{updmap} script to do this:
\begin{verbatim}
updmap --setoption pdftexDownloadBase14 true
\end{verbatim}

Windows users should edit the \texttt{updmap.cfg} files found in their TeX installation directories (one or both
of the following may be present):
\begin{verbatim}
  INSTALLDIR\texmf\web2c\updmap.cfg
  INSTALLDIR\localtexmf\miktex\config\updmap.cfg
\end{verbatim}

Ensure the value for \texttt{pdftexDownloadBase14} is "true," and then follow the instructions found here:
\httpAddr{//docs.miktex.org/manual/} to update your MikTeX installation.

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: Acrobat Distiller}

We recommend to use a Distiller job options file that embeds
all typefaces and does not downsample or subsample images when creating the PDF document.
%------------------------------------------------------------------------
\subsection{Exclusive License Form}

You must include your signed Eurographics Exclusive License Form 
when you submit your finished paper. We MUST have this form before
your paper can be published in the proceedings.

%-------------------------------------------------------------------------
\subsection{Conclusions}

Please direct any questions to the production editor in charge of
these proceedings.

%-------------------------------------------------------------------------

%\bibliographystyle{eg-alpha}
\bibliographystyle{eg-alpha-doi}

\bibliography{egbibsample}

%-------------------------------------------------------------------------
\newpage


\begin{figure*}[tbp]
  \centering
  \mbox{} \hfill
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.3\linewidth]{sampleFig}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.3\linewidth, bb=39 696 126 756]{sampleFig}
  \hfill
  \includegraphics[width=.3\linewidth]{sampleFig}
  \hfill \mbox{}
  \caption{\label{fig:ex3}%
           For publications with color tables (i.e., publications not offering
           color throughout the paper) please \textbf{observe}: 
           for the printed version -- and ONLY for the printed
           version -- color figures have to be placed in the last page.
           \newline
           For the electronic version, which will be converted to PDF before
           making it available electronically, the color images should be
           embedded within the document. Optionally, other multimedia
           material may be attached to the electronic version. }
\end{figure*}

\end{document}


==> EGauthorGuidelines-body_with_teaser.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.02, Jan 25, 2017


\title[EG \LaTeX\ Author Guidelines]%
      {\LaTeX\ Author Guidelines for EUROGRAPHICS Proceedings Manuscripts}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[D. Fellner \& S. Behnke]
{\parbox{\textwidth}{\centering D.\,W. Fellner\thanks{Chairman Eurographics Publications Board}$^{1,2}$\orcid{0000-0001-7756-0901}
        and S. Behnke$^{2}$\orcid{0000-0001-5923-423X} 
%        S. Spencer$^2$\thanks{Chairman Siggraph Publications Board}  
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$TU Darmstadt \& Fraunhofer IGD, Germany\\
         $^2$Graz University of Technology, Institute of Computer Graphics and Knowledge Visualization, Austria
%        $^2$ Another Department to illustrate the use in papers from authors
%             with different affiliations
       } 
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

\teaser{
 \includegraphics[width=\linewidth]{eg_new}
 \centering
  \caption{New EG Logo}
\label{fig:teaser}
}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract}
   The ABSTRACT is to be in fully-justified italicized text, 
   between two horizontal lines,
   in one-column format, 
   below the author and affiliation information. 
   Use the word ``Abstract'' as the title, in 9-point Times, boldface type, 
   left-aligned to the text, initially capitalized. 
   The abstract is to be in 9-point, single-spaced type.
   The abstract may be up to 3 inches (7.62 cm) long. \\
   Leave one blank line after the abstract, 
   then add the subject categories according to the ACM Classification Index 
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see http://www.acm.org/about/class/1998)
% \begin{classification} % according to http:http://www.acm.org/about/class/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
   (see http://www.acm.org/about/class/class/2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010352.10010381</concept_id>
<concept_desc>Computing methodologies~Collision detection</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010588.10010559</concept_id>
<concept_desc>Hardware~Sensors and actuators</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010584.10010587</concept_id>
<concept_desc>Hardware~PCB design and layout</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[300]{Computing methodologies~Collision detection}
\ccsdesc[300]{Hardware~Sensors and actuators}
\ccsdesc[100]{Hardware~PCB design and layout}


\printccsdesc   
\end{abstract}





%-------------------------------------------------------------------------
\section{Introduction}

Please follow the steps outlined in this document very carefully when
submitting your manuscript to Eurographics.

You may as well use the \LaTeX\ source as a template to typeset your own
paper. In this case we encourage you to also read the \LaTeX\ comments
embedded in the document.

%-------------------------------------------------------------------------
\section{Instructions}

Please read the following carefully.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts,
must be kept within a print area %6.31 inches (16.03 cm) 
7 inches (17.7 cm) wide by
%9.10 inches (23.13 cm) 
9.44 inches (24 cm) high. Do not write or print anything
outside the print area. Number your pages on odd sites right
above, on even sites left above, no page number on the first site.
Do not use page numbering within the final version of your paper.


%------------------------------------------------------------------------
\subsection{Formatting your paper}

% All text with the exception of the abstract must be in a two-column format.
% The total allowable width of the text area -- including header and footer
% lines -- is 161\,mm (6.34 inch) wide by 231\,mm (9.10 inch) high.
% 
% Columns are to be 76\,mm (3.0 inch) wide, with a 8\,mm (0.315 inch) space 
% between them.

All text with the exception of the abstract must be in a two-column format.
The total allowable width of the text area -- including header and footer
lines -- is 177\,mm (7 inch) wide by 245\,mm (9.64 inch) high.

Columns are to be 84\,mm (3.3 inch) wide, with a 8\,mm (0.315 inch) space 
between them.

The space between the header line and the first line of the text body and
between the last line of the text body and the footer line is 5\,mm
(0.196 inch) each.
%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If
neither is available on your word processor, please use the font
closest in appearance to Times that you have access to. Only
Type-1 fonts will be accepted.

MAIN TITLE. The title should be in Times 17-point, boldface type and
centered. Capitalize the first letter of nouns, pronouns, verbs, adjectives,
and adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title and
printed in Times 9-point, non-boldface type. This information is to be
followed by two blank lines.

The ABSTRACT ist to be in a one-column format. The MAIN TEXT is to be in a
two-column format.

MAIN TEXT. Type main text in 9-point Times, single-spaced. Do \emph{not} use
double-spacing. All paragraphs should be indented 1 em (the length of the
dash in the actual font). Make sure your text is fully justified -- that is,
flush left and flush right. Please do not place any additional blank lines
between paragraphs. Figure and table captions should be 9-point Times
boldface type as in Figure~\ref{fig:firstExample}.

\noindent Long captions should be set as in Figure~\ref{fig:ex1} or
Figure~\ref{fig:ex3}.

\begin{figure}[htb]
   % an empty figure just consisting of the caption lines
   \caption{\label{fig:ex1}
     'Empty' figure only to serve as an example of long caption requiring 
     more than one line. It is not typed centered but aligned on both sides.}
\end{figure}

\noindent
Figures which need the full textwidth can be typeset as Figure~\ref{fig:ex3}.

\noindent Callouts should be 9-point Times, non-boldface type. Initially
capitalize only the first word of section titles and first-, second-, and
third-order headings.

FIRST-ORDER HEADINGS. (For example, \textbf{1. Introduction}) should be Times
9-point boldface, initially capitalized, flush left, with one blank line
before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, \textbf{2.1. Language}) should be Times
9-point boldface, initially capitalized, flush left, with one blank line
before, and one after. If you require a third-order heading (we discourage
it), use 9-point Times, boldface, initially capitalized, flush left, preceded
by one blank line, followed by a period and your text on the same line.

The headline \emph{(authors / title)} must be shortened if it uses the full 
two column width of the main text.
There must be enough space for the page numbers. Please use ``et al.'' if 
there are more than three authors and specify a shortened version for your title.
%-------------------------------------------------------------------------
\subsection{Footnotes}

Please do \emph{not} use footnotes at all!


%-------------------------------------------------------------------------
\subsection{References}

List all bibliographical references in 9-point Times, single-spaced, at the
end of your paper in alphabetical order. When referenced in the text, enclose
the citation index in square brackets, for example~\cite{Lous90}. Where
appropriate, include the name(s) of editors of referenced books.

For your references please use the following algorithm:
\begin{itemize} 
\item \textbf{one} author: first 3 chars plus year -- 
      e.g.\ \cite{Lous90}
\item \textbf{two}, \textbf{three} or \textbf{four} authors: first char
      of each family name plus year --  e.g.\ \cite{Fellner-Helmberg93} 
      or \cite{Kobbelt97-USHDR} or \cite{Lafortune97-NARF}
\item \textbf{more than 4} authors: first char of family name from 
      first 3 authors followed by a '*' followed by the year -- 
      e.g.\ \cite{Buhmann:1998:DCQ} or \cite{FolDamFeiHug.etal93} 
\end{itemize}

For BibTeX users a style file \ \texttt{eg-alpha.bst} \ is available which
uses the above algorithm.

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.

%%%
%%% Figure 1
%%%
\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.8\linewidth]{sampleFig}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %
  \parbox[t]{.9\columnwidth}{\relax
           For all figures please keep in mind that you \textbf{must not}
           use images with transparent background! 
           }
  %
  \caption{\label{fig:firstExample}
           Here is a sample figure.}
\end{figure}

If your paper includes images, it is very important that they are of
sufficient resolution to be faithfully reproduced.

To determine the optimum size (width and height) of an image, measure
the image's size as it appears in your document (in millimeters), and
then multiply those two values by 12. The resulting values are the
optimum $x$ and $y$ resolution, in pixels, of the image. Image quality
will suffer if these guidelines are not followed.

Example 1: 
%
An image measures 50\,mm by 75\,mm when placed in a document. This
image should have a resolution of no less than 600 pixels by 900
pixels in order to be reproduced faithfully.

Example 2: 
%
Capturing a screenshot of your entire $1024 \times 768$ pixel display
monitor may be useful in illustrating a concept from your research. In
order to be reproduced faithfully, that $1024 \times 768$ image should
be no larger than 85 mm by 64 mm (approximately) when placed in your
document.


%-------------------------------------------------------------------------
\subsection{Color}

\textbf{Please observe:} as of 2003 publications in the proceedings of the
Eurographics Conference can use color images throughout the paper. No
separate color tables are necessary.

However, workshop proceedings might have different agreements! 
Figure~\ref{fig:ex3} is an example for creating color plates.

%------------------------------------------------------------------------
\subsection{Embedding of Hyperlinks / Typesetting of URLs}

Due to the use of the package \texttt{hyperref} the original behavior
of the command $\backslash$\texttt{url} from the package \texttt{url}
is not available. To circumvent this problem we either recommend to
use the command $\backslash$\texttt{httpAddr} from the 
included package \texttt{egweblnk} (see below) or to replace the
command $\backslash$\texttt{url} by the command $\backslash$\texttt{webLink} 
-- e.g. in cases where $\backslash$\texttt{url} has been used
widely in BibTeX-References. In the latter case we suggest to run
BibTeX as usual and then replace all occurences of $\backslash$\texttt{url}  by
$\backslash$\texttt{webLink}

\noindent
The provided commands for hyperlinks, in a nutshell, are:

\begin{description} \itemsep 1ex
\item [\webLinkFont $\backslash$httpAddr \{URL without leading 'http:'\}]
      \mbox{}\\
      e.g. \  \httpAddr{//diglib.eg.org/EG/DL/WS}

\item[\webLinkFont $\backslash$ftpAddr \{URL without leading 'ftp:'\}]
      \mbox{}\\
      e.g. \  \ftpAddr{//www.eg.org/EG/DL/ftpupload}

\item[\webLinkFont $\backslash$URL \{url\}]
      \mbox{}\\
      e.g. \  \URL{http://www.eg.org/EG/DL/WS}

\item[\webLinkFont $\backslash$MailTo \{Email addr\}]
      \mbox{}\\
      e.g. \  \MailTo{publishing@eg.org}

\item[\webLinkFont $\backslash$MailToNA \{emailName\}\{@emailSiteAddress\}]
      \mbox{}\\
      e.g. \  \MailToNA{publishing}{@eg.org}

\item[\webLinkFont $\backslash$webLink\{URL without hyperlink creation\}]
      \mbox{}\\
      e.g. \  \webLink{http://www.eg.org/some_arbitrary_long/but_useless/URL}

\end{description}


%------------------------------------------------------------------------
\subsection{PDF Generation}

Your final paper should be delivered as a PDF document with all typefaces
embedded. \LaTeX{} users should use \texttt{dvips} and \texttt{ps2pdf} to
create this PDF document. Adobe Acrobat Distiller may be used in place of
\texttt{ps2pdf}.

Adobe PDFWriter is \emph{not} acceptable for use. Documents created with
PDFWriter will be returned to the author for revision. \texttt{pdftex} and
\texttt{pdflatex} (and its variants) can be used only if the author can
make certain that all typefaces are embedded and images are not downsampled
or subsampled during the PDF creation process.

Users with no access to these PDF creation tools should make available a
PostScript file and we will make a PDF document from it.


The PDF file \emph{must not} be change protected.

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: dvips / ps2pdf / etc.}

\noindent
\texttt{dvips} should be invoked with the \texttt{-Ppdf} and \texttt{-G0}
flags in order to use Type 1 PostScript typefaces:

\begin{verbatim}
    dvips -t a4 -Ppdf -G0 -o my.ps my.dvi
\end{verbatim}


\noindent
If you are using version 7.x of GhostScript, please use the following method of invoking \texttt{ps2pdf}, in
order to embed all typefaces and ensure that images are not downsampled or subsampled in the PDF
creation process:

\begin{verbatim}
  ps2pdf -dMaxSubsetPct=100 \
         -dCompatibilityLevel=1.3 \
         -dSubsetFonts=true \
         -dEmbedAllFonts=true \
         -dAutoFilterColorImages=false \
         -dAutoFilterGrayImages=false \
         -dColorImageFilter=/FlateEncode \
         -dGrayImageFilter=/FlateEncode \
         -dMonoImageFilter=/FlateEncode \
         mypaper.ps mypaper.pdf
\end{verbatim}


If you are using version 8.x of GhostScript, please use this method in place of the example above:
\begin{verbatim}
  ps2pdf -dPDFSETTINGS=/prepress \
         -dCompatibilityLevel=1.3 \
         -dAutoFilterColorImages=false \
         -dAutoFilterGrayImages=false \
         -dColorImageFilter=/FlateEncode \
         -dGrayImageFilter=/FlateEncode \
         -dMonoImageFilter=/FlateEncode \
         -dDownsampleColorImages=false \
         -dDownsampleGrayImages=false \
         mypaper.ps mypaper.pdf
\end{verbatim}

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: pdftex / pdflatex / etc.}

\noindent
Configuration of these tools to embed all typefaces can be accomplished by editing the \texttt{updmap.cfg} file
to enable inclusion of the standard (or base) 14 typefaces.

Linux users can run the \texttt{updmap} script to do this:
\begin{verbatim}
updmap --setoption pdftexDownloadBase14 true
\end{verbatim}

Windows users should edit the \texttt{updmap.cfg} files found in their TeX installation directories (one or both
of the following may be present):
\begin{verbatim}
  INSTALLDIR\texmf\web2c\updmap.cfg
  INSTALLDIR\localtexmf\miktex\config\updmap.cfg
\end{verbatim}

Ensure the value for \texttt{pdftexDownloadBase14} is "true," and then follow the instructions found here:
\httpAddr{//docs.miktex.org/manual/} to update your MikTeX installation.

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: Acrobat Distiller}

We recommend to use a Distiller job options file that embeds

all typefaces and does not downsample or subsample images when creating the PDF document.
%------------------------------------------------------------------------
\subsection{Exclusive License Form}

You must include your signed Eurographics Exclusive License Form 
when you submit your finished paper. We MUST have this form before
your paper can be published in the proceedings.

%-------------------------------------------------------------------------
\subsection{Conclusions}

Please direct any questions to the production editor in charge of
these proceedings.

%-------------------------------------------------------------------------

%\bibliographystyle{eg-alpha}
\bibliographystyle{eg-alpha-doi}

\bibliography{egbibsample}

%-------------------------------------------------------------------------
\newpage


\begin{figure*}[tbp]
  \centering
  \mbox{} \hfill
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.3\linewidth]{sampleFig}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.3\linewidth, bb=39 696 126 756]{sampleFig}
  \hfill
  \includegraphics[width=.3\linewidth]{sampleFig}
  \hfill \mbox{}
  \caption{\label{fig:ex3}%
           For publications with color tables (i.e., publications not offering
           color throughout the paper) please \textbf{observe}: 
           for the printed version -- and ONLY for the printed
           version -- color figures have to be placed in the last page.
           \newline
           For the electronic version, which will be converted to PDF before
           making it available electronically, the color images should be
           embedded within the document. Optionally, other multimedia
           material may be attached to the electronic version. }
\end{figure*}

\end{document}


==> sections/01_introduction.tex <==
\section{Introduction}
%The increasing demand of computer generated natural human motion for many industrial, as well as, entertainment applications, coupled with the decreasing cost of motion capture production, are a driving force for more sophisticated tools to process and analyze motion capture data. However, many of these applications, like motion retargeting \cite{??} or gesture recognition \cite{??}, require small,  semantically similar pieces of motion data in order to function properly \cite{bouchard2008automated}. Typical motion capture sessions, however, produce long streams of motion. Naturally, a preprocessing step is needed to break the motion stream up into short pieces, which are semantically meaningful for the application. So far, this process is often done manually, which is laborious and time consuming.

%To reduce time and effort, an automatic solution is needed. Such an algorithm would segment motion capture data into a collection of smaller contiguous portions of the original data. Another factor is to incorporate semantic meaning into these motion pieces to be able to synthesize new motions of the same motion type. Thus, high-level descriptive labels are needed for such tasks. In kinematic segmentation, segment labels are akin to a low-level kinematic description of a motion, like \emph{high velocity sagittal motion} \cite{bouchard2007semantic}. This makes the labels harder to interpret and less intuitive to work with. Whereas semantic segmentation uses high-level descriptions, such as \emph{carrying a package}, to label the resulting segments, which accounts for more intuitiveness. Hence, one of the main goals of automatic motion segmentation should be to produce semantically sophisticated labels of motion segments on a general set of actions. 

%Additionally, manual segmentation is often coupled with personal bias, thus producing different results with each person or even with each attempt of the same person and the same data. An automatic algorithm overcomes these inter- and intra-annotator disagreements by producing the same output when the same input is given to the system, making it deterministic.

%TODO: Write section about outline of this paper...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Nosh new
There is an increasing demand for computer-generated natural human motion for many industrial applications ranging from ergonomics analysis to entertainment applications. The decreasing costs of motion capture devices and recent developments in the area of motion synthesis have lead to motion models incorporating large motion capture databases to a single motion model (e.g. \cite{Du:2016:SFP:2994258.2994277, holden2017phase, zhang2018MANN, min2012motion}). Semantic segmentation of motion capture data is a necessary pre-processing step required by many data-driven motion synthesis solutions. Given a motion capture sequence, the goal is to simultaneously segment every action in time in a fine-grained manner and classify each constituent segment. 

% Janis: 
%There is an increasing demand for computer-generated natural human motion for many industrial applications ranging from ergonomics analysis to entertainment applications. The decreasing costs of motion capture devices and recent developments in the area of motion synthesis have lead to motion models incorporating large motion capture databases to a single motion model (e.g. \cite{Du:2016:SFP:2994258.2994277, holden2017phase, zhang2018MANN}). Labeling of motion capture data is a necessary pre-processing step required by many data-driven motion synthesis solutions. Given a heterogeneous motion capture sequence, the task is to densely segment the whole sequence in semantically similar pieces in a fine-grained manner. 
% Old remove if reviewed:
%The increasing demand of computer generated natural human motion for many industrial, as well as, entertainment applications, coupled with the increasing cost of motion capture production, are a driving force for models to generate new variations of natural-looking controllable human motion. However, many of these models, like \cite{min2012motion}, \cite{holden2017phase} rely on small, semantically similar pieces of motion data in order to function properly \cite{bouchard2008automated}. This is due to the fact that modeling a motion stream which is heterogeneous in nature (i.e. it consists of various actions and sub-actions) is inefficient \cite{}. Typical motion capture sessions, however, produce long streams of motion. Naturally, a pre-processing step is needed to break the motion stream up into short pieces, which are semantically meaningful for the application. 
%OLD   remove if reviewed!: 
%So far, this process is often done manually, which is laborious and time consuming.
% New Nosh:
Manual segmentation is laborious, time-consuming and, most of all, subjective due to inter- and intra-annotator disagreements. An automatic algorithm overcomes disagreements by consistently producing a deterministic output. 
Kinematic-based segmentation approaches \cite{jenkins2003automated, muller2005efficient, fod2002automated} tackle this problem by comparing low-level handcrafted time-series features to extract the segment boundaries. Such approaches are computationally fast but require manually designing features for different motion types. Data-analysis-based segmentation approaches \cite{barbivc2004segmenting, lv2006recognition, muller2006motion} overcome this problem by making use of unsupervised machine learning techniques. While these are able to learn a high-level feature space and able to generalize to new motions, they generally cannot make any insights on the content or semantics of the motion. Hence, semantic labels are difficult to obtain from such models. Therefore, we focus exclusively on recognition-based segmentation methods \cite{kahol2004automated, wu2014leveraging, du2015hierarchical} in this work. These methods are based on supervised machine-learning techniques and can learn a high-level feature space (in contrast to the hand-crafted features from the kinematic-based approaches), while simultaneously attaining insights on the content of the motion data making semantic segmentation possible. Current state-of-the-art recognition-based models make use of temporal classifiers to extract motion segments. Such temporal models have been limited to sliding window action detectors \cite{rohrbach2016recognizing, singh2016multi, ni2016progressively}, which typically do not capture long-range temporal patterns or recurrent models \cite{lstm, singh2016multi} which can capture latent temporal patterns but are difficult to train \cite{pascanu2013difficulty}.

% Janis:
%Manual segmentation is laborious, time-consuming and, most of all, subjective. An automatic algorithm overcomes these inter- and intra-annotator disagreements by consistently producing a deterministic output. It segments an input motion stream into a collection of smaller segments. Incorporating semantic meaning into each segment enables a subsequent process to synthesize new motions of the same type. These descriptive frame labels can differ in their granularity. 
%In kinematic segmentation, frame labels are akin to a low-level kinematic description of a motion, like \emph{high velocity sagittal motion} \cite{bouchard2007semantic}. This makes the labels harder to interpret and less intuitive to work with. Semantic segmentation, on the other hand, uses high-level descriptions, such as \emph{reaching for an object}, to label the frames, which accounts for more intuitiveness. These high-level descriptions are required to model specific motion primitives (e.g. \emph{left-stance}, \emph{right-stance},...) \cite{min2012motion, Du:2016:SFP:2994258.2994277} or controllable actions (e.g. \emph{walking, running, jumping}...) \cite{zhang2018MANN, holden2017phase}. 

%Old   remove if reviewed!:
%To reduce time and effort, an automatic solution is needed. Such an algorithm would automatically segment an input motion stream into a collection of smaller pieces while incorporating semantic meaning into these pieces to be able to synthesize new motions of the same type. Thus, high-level descriptive frame labels are needed for such tasks. In kinematic segmentation, frame labels are akin to a low-level kinematic description of a motion, like \emph{high velocity sagittal motion} \cite{bouchard2007semantic}. This makes the labels harder to interpret and less intuitive to work with. Whereas semantic segmentation uses high-level descriptions, such as \emph{reaching for an object}, to label the frames, which accounts for more intuitiveness. Hence, one of the main goals of automatic motion segmentation should be to produce semantically-meaningful labels for motion frames on a general set of actions. 
%Additionally, manual segmentation is often subjective, thus producing different results with each person or even with each attempt of the same person and the same data. An automatic algorithm overcomes these inter- and intra-annotator disagreements by producing the same output when the same input is given to the system, making the outcome deterministic.

% New Nosh
In this paper, we discuss a recently proposed class of time-series models based on Convolutional Neural Network models, which is able to capture long-range dependencies more efficiently. Such networks have been coined the term Temporal Convolutional Networks (TCNs) \cite{lea2016temporal, bai2018empirical}. Recent studies \cite{bai2018empirical, Lea2017TemporalCN} have shown that such networks exhibit longer memories than recurrent architectures, which are supposed to have ``infinite memory" \cite{bai2018empirical, lstm}, by applying a hierarchy of temporal filters. We present a type of TCN which can be used for fine-grained semantic segmentation of motion capture data. Our Dilated Temporal Fully-Convolutional Network (DT-FCN) takes inspiration from image segmentation models using Fully-Convolutional Neural Networks (FCN) \cite{long2015fully, yu2015multi} and TCN-based sequential models \cite{bai2018empirical, wavenet, lea2016temporal} for time-dependant data. The DT-FCN makes use of acausal dilated temporal convolutions to capture long-range dependencies due to the increased receptive field size obtained by the dilation. We apply it on motion data which we represent as images. Thus the first layer consists of a 2D temporal convolution layer. In this task we segment fine-grained motion primitives (i.e. \emph{left step}, \emph{right step} etc.) used for motion modeling tools \cite{min2012motion} from motion data.
We compare our model against two state-of-the-art TCN-based action segmentation models (Encoder-Decoder TCN \cite{lea2016temporal} and DilatedTCN \cite{Lea2017TemporalCN}) and a popular LSTM-based sequential model (Bidirectional LSTM \cite{graves2005framewise, lstm}) and outperform them in terms of accuracy as well as robustness towards highly noisy data. 

%Janis:
%We designed a neural network model, capable of automatically generating semantic frame labels for a vast variety of actions inside the motion stream. This model requires only a small amount of previously-annotated human motion capture data as a training set. While a great deal of work has been done on semantic image segmentation using neural networks, there is little work on semantic motion segmentation to our knowledge. Hence we transformed the problem of motion sequence segmentation to an image segmentation problem, to benefit from the recent advances in this area. We are generating a database of 2D RGB images from our motion capture database of articulated joint rotations and positions, based on the work of \cite{laraba20173d, ke2017new}. Thus we can apply neural networks for image segmentation on these \emph{motion images} to generate a dense segmentation of the original motion clip. 

% old remove if reviewed!:
%Given a small dataset of previously-annotated human motion capture data based on their corresponding semantic segment, we came up with a neural network model that automatically generates the semantic frame labels corresponding to segments for any input motion stream. While a great deal of work has been done on semantic image segmentation using neural networks, there is little work on semantic motion segmentation to our knowledge. As a result, to benefit from the advances in image segmentation using neural networks, we came up with the idea to pose our motion segmentation problem as an image segmentation one by generating a database of 2D RGB images from our motion capture database based on the work \cite{motion to RGB} to be used further for image segmentation. 

%new Janis:
%However, there is a difference between traditional image and motion image segmentation, which roots from the intrinsic temporal property of motion data. Traditional image segmentation is performed over two spatial dimensions of an image. Motion data, however, consists of Cartesian joint positions over time, thus the generated motion images \cite{laraba20173d, ke2017new} have a spatial and a temporal dimension. As semantic segmentation of motions is supposed to create estimations in the temporal domain, the motion image segmentation should only predict labels for one image dimension. Additionally, motion sequences are varying in length and consequently, the motion images vary in size. This makes the motion images more challenging to handle. 

%To tackle these issues, we propose a novel architecture (compare Figure \ref{fig:model_overview}), which is inspired by both, advances in image segmentation methods \cite{long2015fully} and sequence modeling \cite{bai2018empirical}. The contribution of the paper can be summarized to the following: 

%old   remove if reviewed!: 
%However, there is a difference between image and motion image segmentation tasks which roots from the intrinsic temporal property of motion data. That is, image segmentation is performed over two spatial dimensions of an image while a motion image \cite{motion to RGB} obtained by Cartesian values of joints over time consists of spatial vs. temporal domains, and our goal is to perform segmentation only over the temporal domain. Additionally, our motion sequences come in different lengths which makes it challenging to handle.  To tackle these issues we propose the architecture in Figure 8 which is inspired by both advances in image segmentation methods \cite{FCN} and sequence modeling \cite{ED-TCN}. 

%Old. Remove if reviewed! 
%The contribution of our proposed model can be summarized to the following: 
%\begin{itemize}
%    \item Creating a database of 2D RGB images that are obtained from our motion capture database used for motion image segmentation. 
%    \item Proposing a CNN-based architecture which performs convolutions only in temporal domain to enable extracting only temporal dependencies that is suitable for motion segmentation task. 
%    \item Using the concept of Fully-Convolutional networks for being able to handle input motion sequences of different lengths. 
%    \item Using the concept of Dilated Convolutions that enables us to increase the receptive field size of our network at a much lower cost than traditional convolutions in terms of number of parameters.  
%\end{itemize}

In the remainder of this work we first discuss most of the related work on kinematic and semantic motion segmentation as well as data-driven motion synthesis as the targeted application field in Section 2. We then explain the procedure of converting our motion capture sequences to 2D RGB images in Section 3. In Section 4 we provide a comprehensive overview of our network architecture and its different building blocks and functionalities. Section 5 consists of our data-set explanation, the implementation details and evaluation results. Finally in Section 6 we provide a summary, conclusion and further outlook of this work.

% old. remove if reviewed:
%In the remainder of this work we first discuss most of the related work on kinematic and semantic motion segmentation and one of its major applications that is data-driven motion synthesis in Section 2. We then explain the procedure of converting our motion capture sequences to 2D RGB images in Section 3. In Section 4. we provide a comprehensive overview of our network architecture called Dilated Fully-Convolutional Network and its different building blocks and functionalities. Section 5. consists of our dataset explanation, the implementation details and evaluation results of our method and a comparison with different benchmark methods. Finally in Section 6 we give a summary of this work and provide some conclusions about it.






==> sections/02_background.tex <==
\section{Background}
\subsection{Data-driven Motion Synthesis}
% Janis + Han
A recent overview of motion synthesis approaches can by found by Guo et al. \cite{guo2015adaptive}. Data-driven motion synthesis for digital human models has been widely used to generate realistic and natural human motion. Many data-driven techniques require motion segmentation as a necessary pre-processing step, for instance, statistical modeling approaches \cite{taylor2010convolutional,min2009interactive,min2012motion} and graph-based approaches \cite{kovar2002motion,lee2002motion, kovar2008motion}. For semantic-embedded motion synthesis \cite{min2012motion,du2016joint}, recorded motions need to be split in structurally- and semantically- similar segments. An action can then be represented as a finite set of semantic-embedded states (motion primitives). For instance, a normal walking can be decomposed as a combination of left and right steps \cite{min2012motion}. 

% Fig. \ref{fig:graph} illustrates the morphable graph, where nodes are named motion primitives, which represent the similar motion segments and edges are the transitions between motion primitives.

% old version from Han: remove if reviewed
%Recently, data-driven motion synthesis for digital human models has been widely used to generate realistic and natural human motion. A recent overview of motion synthesis approaches can by found by Guo et al. \cite{guo2015adaptive}. Many data-driven motion synthesis techniques require motion segmentation as a necessary pre-processing step, for instance, statistical modeling approaches \cite{taylor2010convolutional,min2009interactive,min2012motion} and graph-based approaches \cite{kovar2002motion,lee2002motion, kovar2008motion}. For semantic-embedded motion synthesis \cite{min2012motion,du2016joint}, recorded motions need to be split in structurally- and semantically- similar segments.Fig. \ref{fig:graph} illustrates the morphable graph, where nodes are named motion primitives, which represent the similar motion segments and edges are the transitions between motion primitives.

% Old Version: remove if reviewed
%Recently, data-driven motion synthesis for digital human models has been widely used to generate realistic and natural human motion. Many data-driven motion synthesis techniques require fine-grained segmented motion primitives (such as \emph{left step} and \emph{right step}) as a pre-processing step (e.g. \emph{Motion Graphs++} \cite{min2012motion}). A recent overview of motion synthesis approaches can by found by Guo et al. \cite{guo2015adaptive}. In most of these approaches the motion recordings need to be split in structurally-similar segments for further statistical \cite{taylor2010convolutional,min2009interactive,min2012motion} and/or graph-based \cite{kovar2002motion,lee2002motion} modeling. Interactive applications, such as video games, control their animation often through motion graphs \cite{min2012motion, kovar2008motion, du2016joint}, where nodes are motion segments and the transitions represent potential segment sequencing. Such a graph is often created by using semantic segments of motion capture data with smooth transitions to all other potential segments. A morphable graph model \cite{min2012motion} used in these applications is shown Fig. \ref{fig:graph}. Each graph node is a generative statistical model.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{images/mograph1.png}
%     \includegraphics[width=0.4\linewidth]{images/mograph2.png}
%     \caption{Left: Morphable graphs model for running \cite{min2012motion} with motion primitives ``left stance'', ``flight 1'', ``right stance'' and ``flight 2''. Right: Different running styles generated by this motion synthesis model \cite{min2012motion}.}
%     \label{fig:graph}
% \end{figure}

\subsection{Motion and Action Recognition and Segmentation}
% Janis + Han
To our knowledge there is not extensive work done in motion primitive segmentation (i.e. segmenting \emph{left step} from \emph{right step} for example) using recognition-based segmentation methods, therefore most of the mentioned related work focuses on action segmentation (i.e. segmenting \emph{walking} from \emph{picking}). We include work based on 3D motion capture data, as well as, 2D video based data. Similar to Bouchard \cite{bouchard2008automated}, we divide existing algorithms into three major types of motion segmentation methods. These are \emph{(i) kinematic-based}, \emph{(ii) data analysis-based}, and \emph{(iii) recognition-based segmentation}.

% old Han,  remove if reviewed
% Similar to Bouchard \cite{bouchard2008automated}, we divide existing algorithms into three major types of motion segmentation methods, in addition to manual segmentation. The other three being \emph{(i) kinematic-based segmentation}, \emph{(ii) data analysis-based segmentation}, and \emph{(iii) recognition-based segmentation}. To our knowledge there is not extensive work done in motion primitive segmentation (i.e. segmenting \emph{left step} from \emph{right step} for example), therefore most of the mentioned related work focuses on action segmentation (i.e. segmenting \emph{walking} from \emph{picking}). We include work based on 3D motion capture data, as well as, 2D video based data.

% Old.  remove if reviewed
%Similar to Bouchard \cite{bouchard2008automated}, we divide existing algorithms into three major types of motion segmentation methods, in addition to manual segmentation. The other three being \emph{(i) kinematic-based segmentation}, \emph{(ii) data analysis-based segmentation}, and \emph{(iii) recognition-based segmentation}. To our knowledge there is not extensive work done in motion primitive segmentation (i.e. segmenting \emph{left step} from \emph{right step} for example), therefore most of the mentioned related work focuses on action segmentation (i.e. segmenting \emph{walking} from \emph{picking}). We include work based on 3D motion capture data, as well as, 2D video based data.

% Han
%\textbf{Kinematic-based segmentation.} Kinematic segmentation is segmentation based on low-level kinematic features such as euclidean coordinates or rotational velocity of joints. Commonly, the segmentation is accomplished by comparing hand-crafted, low-level kinematic time series features to determine the patterns in the feature data that correlate to segment boundaries. Segments for new motion capture data are then found by computing the same time series features and searching for the correlated segment boundary patterns. These methods often require manually setting parameters to determine how similar two segments are to one another. Min et al. \cite{min2012motion} and Holden et al. \cite{holden2017phase} use coordinate based contact point measures to classify motion primitives in motion capture data, e.g. distance between foot and floor. A similar position based method is used by Jenkins and Matari\'c \cite{jenkins2003automated, jenkins2004spatio} using an arm's centroid to segment arm motions. Fod et al. \cite{fod2002automated} implement two different approaches for motion capture data segmentation of an arm based on zero-crossings in angular velocity in different degrees of freedom in the arm. M\"uller et al. \cite{muller2005efficient} use boolean features per joint which indicate the spatial relationship between a joint and a plane formed by other joints and a joint angle's or velocity's relationship to a threshold.  A sudden change in direction correlates with reaching a destination and the end of a motion. Zhao and Badler \cite{zhao2005acquiring} calculate segment boundaries when hand linear acceleration zero crosses and curvature is above some threshold.

% New nosh

\textbf{Kinematic-based segmentation.} Kinematic segmentation is segmentation based on low-level kinematic features such as euclidean coordinates or rotational velocity of joints. Commonly, the segmentation is accomplished by comparing hand-crafted, low-level kinematic time series features to determine the patterns in the feature data that correlate to segment boundaries. Segments for new motion capture data are then found by computing the same time series features and searching for the correlated segment boundary patterns. These methods often require manually setting parameters to determine how similar two segments are to one another. Min et al. \cite{min2012motion} and Holden et al. \cite{holden2017phase} use coordinate based contact point measures to classify motion primitives in motion capture data, e.g. distance between foot and floor to determine a step. A similar position based method is used by Jenkins and Matari\'c \cite{jenkins2003automated, jenkins2004spatio} using an arm's centroid to segment arm motions. Fod et al. \cite{fod2002automated} implement two different approaches for motion capture data segmentation of an arm based on zero-crossings in angular velocity in different degrees of freedom in the arm. M\"uller et al. \cite{muller2005efficient} use boolean features per joint which indicate the spatial relationship between a joint and a plane formed by other joints and a joint angle's or velocity's relationship to a threshold.  A sudden change in direction correlates with reaching a destination and the end of a motion. Zhao and Badler \cite{zhao2005acquiring} calculate segment boundaries when hand linear acceleration zero crosses and curvature is above some threshold. Since such low-level features have to be designed separately for each new task, kinematic-based segmentation methods are unfit for segmenting a multitude of different actions.

% Old,  remove if reviewed
%\textbf{Kinematic-based segmentation.} Kinematic segmentation is segmentation based on low-level kinematic features such as euclidean coordinates or rotational velocity of joints. Commonly, the segmentation is accomplished by comparing hand-crafted, low-level kinematic time series features to determine the patterns in the feature data that correlate to segment boundaries. Segments for new motion capture data are then found by computing the same time series features and searching for the correlated segment boundary patterns. These methods often require manually setting parameters to determine how similar two segments are to one another. Min et al. \cite{min2012motion} and Holden et al. \cite{holden2017phase} use coordinate based contact point measures to classify motion primitives in motion capture data, e.g. distance between foot and floor. A similar position based method is used by Jenkins and Matari\'c \cite{jenkins2003automated, jenkins2004spatio} using an arm's centroid to segment arm motions. Fod et al. \cite{fod2002automated} implement two different approaches for motion capture data segmentation of an arm based on zero-crossings in angular velocity in different degrees of freedom in the arm. M\"uller et al. \cite{muller2005efficient} use boolean features per joint which indicate the spatial relationship between a joint and a plane formed by other joints and a joint angle's or velocity's relationship to a threshold.  A sudden change in direction correlates with reaching a destination and the end of a motion. Zhao and Badler \cite{zhao2005acquiring} calculate segment boundaries when hand linear acceleration zero crosses and curvature is above some threshold.

%Han
\textbf{Data-analysis-based segmentation.} 
In order to automatically find features for segmentation, many unsupervised data analysis methods have been proposed. Barbi\v{c} et al. \cite{barbivc2004segmenting} shows impressive results using three different algorithms based on Principle Component Analysis (PCA), Probabilistic PCA, and Gaussian Mixture Models (GMM). Lee and Elgammal \cite{lee2006human} use $k$-means \cite{lloyd1982least} to estimate the GMM that corresponds to a cluster of a motion primitive. A more sophisticated approach by Zhou et al. \cite{zhou2008aligned, zhou2013hierarchical} uses the $k$-means algorithm with a kernel extension \cite{scholkopf1998nonlinear} for temporal clustering of data to segment actions. Each cluster denotes an action class. Another method introduced by M\"uller et al. \cite{muller2006motion} makes use of so-called Motion Templates (MT) that consist of a set of predefined dynamically time-warped binary pose features. Classification and segmentation are done via template matching. Many variants of motion features \cite{laraba20173d, wu2014leveraging, lv2006recognition} are proposed to provide a more informative representation for motion capture data. These methods are able to learn distinct high-level features from the data and automatically segment motions based on these features. Hence, in comparison to kinematic-based segmentation, they produce more sophisticated results and can be used for unseen data. However, data-analysis-based approaches are generally lacking control of the feature selection and are generally not able to produce semantic labels as they are not able to make any insights on the content or semantics of the motion data.


%Old,  remove if reviewed
%\textbf{Data-analysis-based segmentation.} The next class of segmentation methods draws from data analysis methods, such as time series analysis \cite{??}, Principle Component Analysis (PCA) \cite{pearson1901liii}, Gaussian distribution models \cite{??} and other unsupervised machine learning algorithms, such as clustering \cite{lloyd1982least}. These methods are highly data-driven and are able to learn or correlate distinct high-level features from the data itself and automatically segment motion based on these features. Hence, in comparison to kinematic based segmentation, they produce more sophisticated results. A consequence of this is that they are computationally less efficient, in contrast to the kinematic segmentation methods. The main advantage of data analysis based methods, however, is that they do not require manually labeled data to achieve reasonable results. Hence, they can are able to generalize to unseen motions without having to come up with new hand-crafted features. Nevertheless, a major disadvantage of such methods is the lack of control of what is supposed to be learned for a specific motion segmentation task as they are not able to make any insights on the content or semantics of the motion data. Furthermore, these methods are not able to produce semantic annotations, which would be useful for many motion synthesis tasks where specific motions might be needed. One of the earliest works on motion capture segmentation by Barbi\v{c} et al. \cite{barbivc2004segmenting} shows impressive results using three different algorithms based on PCA, Probabilistic PCA and Gaussian Mixture Models (GMM) \cite{??}, respectively. Lee and Elgammal \cite{lee2006human} use $k$-means \cite{lloyd1982least} to estimate the GMM that corresponds to a cluster of a motion primitive. A more sophisticated approach by Zhou et al. \cite{zhou2008aligned, zhou2013hierarchical} uses the $k$-means algorithm with a kernel extension \cite{scholkopf1998nonlinear} for temporal clustering of data to segment actions. Each cluster denotes an action class. Another method introduced by M\"uller et al. \cite{muller2006motion} makes use of so-called Motion Templates (MT), which consist of a set of predefined dynamically time warped binary pose features. Classification and segmentation of motion capture data is then done via template matching. Many variants of motion features \cite{laraba20173d, wu2014leveraging, lv2006recognition} are proposed to provide a more informative representation for motion capture data.

% Han
\textbf{Recognition-based segmentation.}
Recognition-based segmentation is based on supervised learning. Typically, in supervised motion segmentation techniques a collection of motion capture data is manually segmented and labeled to train a classifier. Therefore, the created segments by the classifier can be as complex as the ones segmented by humans. Kahol et al. \cite{kahol2004automated} use a na\"ive Bayesian classifier to derive choreographer segmentation profiles from dance motion capture sequences. This makes these techniques compelling for segmentation tasks for motion synthesis. Bouchard and Badler \cite{bouchard2007semantic, bouchard2015segmenting} have proposed to our knowledge the first neural network-based segmentation method on motion capture data. They perform Laban Movement Analysis (LMA) \cite{levy2003use} to obtain more meaningful features than simple kinematic features. These features are then used to train 121 perceptrons for segment boundary detection. In recent years, deep learning methods have gained popularity over such more shallow networks. An approach by Wu et al. \cite{wu2014leveraging} uses Hidden Markow Model (HMM) to model the sequential dynamics of motion capture data and adopt a multi-layer neural network to train the emission probabilities from hidden action states to observed pose sequences. Their approach does not require hand-crafted features and can achieve competitive results on the MSR Action3D \cite{li2010action} and MSRC-12 \cite{fothergill2012instructing} motion data sets for high-level action recognition and segmentation. Recurrent neural network (RNN) methods (e.g. \cite{fragkiadaki2015recurrent, singh2016multi}) have exclusively been developed for sequence modeling tasks, like the temporal segmentation of motion capture or video data. Well-regarded books \cite{goodfellow2016deep} and courses \cite{CourseraSequence} on sequential learning focus almost exclusively on RNNs. Fragkiadaki et al. \cite{fragkiadaki2015recurrent} have proposed a three-layered encoder-decoder model based on recurrent neural networks for human pose estimation in video data. To overcome the vanishing gradient problem \cite{hochreiter1991untersuchungen, hochreiter2001gradient} in RNNs, Long Short-Term Memory (LSTM) networks \cite{lstm} are used instead for ``memorizing'' very long sequences.
Du et al. \cite{du2015hierarchical} propose a multi-layered LSTM for action recognition that feeds skeleton data into five sub networks for different body parts at the initial layer and hierarchically fuses the output in higher layers. With this they are able to achieve state-of-the-art results in action recognition on the MSR Action3D \cite{li2010action}, Berkeley MHAD \cite{ofli2013berkeley} and HDM05 \cite{muller2007documentation} data sets. 
However, the major disadvantage of RNNs is a difficult and slow training procedure. Recent studies \cite{bai2018empirical} suggest that certain architectures of Convolutional Neural Networks (CNNs) \cite{wavenet, kalchbrenner2016neural, dauphin2016language, gehring2017convolutional}, which are traditionally used for image classification, can reach state-of-the-art results in typical sequence modeling tasks such as word translation or audio synthesis.
Bai et al. \cite{bai2018empirical} have conducted an extensive study about Temporal Convolutional Networks (TCNs) outperforming different types of RNNs, including LSTM and Gated Recurrent Units \cite{chung2014empirical} in various sequence modeling tasks. They further study long-range information propagation in convolutional and recurrent networks, and show that the ``infinite memory'' advantage of LSTMs is largely absent in practice. They show that TCNs exhibit longer memory than recurrent architectures with the same capacity. TCNs have also been used for action segmentation. Lea et al. \cite{lea2016temporal, rene2017temporal} use an Encoder-Decoder TCN and a variation of WaveNet \cite{wavenet} to segment different actions from the 50 Salads \cite{stein2013combining}, MERL Shopping \cite{singh2016multi} and GTEA \cite{fathi2011learning} video datasets. In order to apply CNNs also on action recognition tasks with motion data, Laraba et al. \cite{laraba20173d} propose a conversion of skeleton sequences into RGB images. Similarly, Ke et al. \cite{ke2017new} process skeleton sequences into a set of images, each representing the entire skeleton sequence with a focus on one particular spatial relationship, and apply a convolutional Multi-Task Learning Network architecture for segmentation. We explore a similar strategy to Laraba et al. \cite{laraba20173d, ke2017new} and incorporate results of Bai et al. \cite{bai2018empirical, rene2017temporal} on fine-grained motion segmentation tasks with motion capture data. Our model draws inspiration from common image segmentation methods \cite{long2015fully}, as well as recent advances in sequences modeling \cite{bai2018empirical}.

% Old,  remove if reviewed
%\textbf{Recognition-based segmentation.} This class of segmentation techniques is based on supervised machine learning recognition techniques. Supervised learning techniques have the advantage that the created segments can be as complex as manual segmentation, due to the manual labeling of the training data. Typically, a collection of motion capture data is manually segmented and labeled and used to train a classifier. While these methods are difficult to implement for general or unknown motion types and the initial labeling still requires tedious human labor, they provide high flexibility and control when it comes to motion segmentation. The granularity of the segmentation result can be decided by the annotator of the training data. This flexibility and the ability to have a controlled output, makes these techniques compelling for segmentation tasks for motion synthesis. Kahol et al. \cite{kahol2004automated} use a na\"ive Bayesian classifier to derive choreographer segmentation profiles from dance motion capture sequences. Bouchard and Badler \cite{bouchard2007semantic, bouchard2015segmenting} have proposed to our knowledge the first neural network-based segmentation method on motion capture data. They perform Laban Movement Analysis (LMA) \cite{levy2003use} to obtain more meaningful features than simple kinematic features. These features are then used to train 121 perceptrons for segment boundary detection. In recent years, deep learning methods have gained popularity over such more shallow networks. An approach by Wu et al. \cite{wu2014leveraging} uses a Hidden Markow Model to model the sequential dynamics of motion capture data and adopt a multi-layer neural network to train the emission probabilities from hidden action states to observed pose sequences. Their approach does not require hand crafted features and can achieve competitive results on the MSR Action3D \cite{li2010action} and MSRC-12 \cite{fothergill2012instructing} motion data sets for high-level action recognition and segmentation. Recurrent neural network (RNN) methods \cite{??} have exclusively been developed for sequence modeling tasks, like the temporal segmentation of motion capture or video data. Well-regarded books \cite{goodfellow2016deep} and courses \cite{ng2018coursera Course 5 of Deep Learning Specialization} on sequential learning focus almost exclusively on RNNs. Fragkiadaki et al. \cite{fragkiadaki2015recurrent} have proposed a three layered encoder-decoder model based on recurrent neural networks to do human pose estimation in video data based on motion capture data for training and synthesis. To overcome the vanishing gradient problem \cite{??} in RNNs, Long Short-Term Memory (LSTM) networks \cite{lstm} are used instead for ``memorizing'' very long sequences. Du et al. \cite{du2015hierarchical} propose a multi-layered LSTM network for action recognition that feeds skeleton data into five sub networks for different body parts at the initial layer and hierarchically fuses the output in higher layers. With this they are able to achieve state-of-the-art results in action recognition on the MSR Action3D \cite{li2010action}, Berkeley MHAD \cite{ofli2013berkeley} and HDM05 \cite{muller2007documentation} data sets. As convincing as these applications may appear in terms of recognition and the complexity of features recurrent models are able to learn, one of their major disadvantages is that their training is extremely difficult and slow \cite{bai2018empirical}. Due to their sequential nature, one training step has to be finished before another can start as the next training step is based on the output of the previous step. This makes parallelization during training tough in comparison to other neural network models \cite{cnn, dense networks} which are easy to parallelize. Furthermore, the vanishing and exploding gradient problem \cite{??} in recurrent architectures makes training on very long sequences a challenging task. Recent studies suggest that certain architectures of Convolutional Neural Networks (CNNs) \cite{wavenet, kalchbrenner2016neural, dauphin2017language, gehring2017convolutional}, which are traditionally used for image classification, can reach state-of-the-art results in typical sequence modeling tasks such as word translation or audio synthesis. Bai et al. \cite{bai2018empirical} have conducted an extensive study about Temporal Convolutional Networks (TCNs) outperforming different types of RNNs, including LSTM and Gated Recurrent Units \cite{??} in various sequence modeling tasks. They further study long-range information propagation in convolutional and recurrent networks, and show that the ``infinite memory'' advantage of LSTMs is largely absent in practice. They show that TCNs exhibit longer memory than recurrent architectures with the same capacity. TCNs have also been used for action segmentation. Lea et al. \cite{lea2016temporal, rene2017temporal} use an Encoder-Decoder TCN and a variation of WaveNet \cite{wavenet} to segment different actions from the 50 Salads \cite{??}, MERL Shopping \cite{??} and GTEA \cite{??} video datasets. In order to apply CNNs also on action recognition tasks with motion data, Laraba et al. \cite{laraba20173d} propose a conversion of skeleton sequences into RGB images, where the color  of a pixel represents the normalized position of a joint at a certain frame. Similarly, Ke et al. \cite{ke2017new} process skeleton sequences into a set of images, each representing the entire skeleton sequence with a focus on one particular spatial relationship, and apply a convolutional Multi-Task Learning Network architecture for segmentation. We explore a similar strategy to Laraba et al. \cite{laraba20173d, ke2017new} and incorporate results of Bai et al. \cite{bai2018empirical, rene2017temporal} on fine-grained motion segmentation tasks with motion capture data. Our model draws inspiration from common image segmentation methods \cite{long2015fully}, as well as recent advances in sequences modeling \cite{bai2018empirical}. 

==> sections/03_motion_images.tex <==
\section{Motion Image Generation}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/mixed_29_described.png}
    \caption{Sample generated motion image from local XYZ joint position coordinates. Each columns represents a frame in the motion capture sequence, while each row the XYZ joint locations in RGB space. The image is then scaled vertically to a fixed height using bi-cubic interpolation.}
    \label{fig:motion_image_mixed}
\end{figure}

%In order to be able to turn a motion segmentation problem into an image segmentation one, we first transform our motion capture data to an RGB image domain, much in the spirit of \cite{laraba20173d, ke2017new}. A motion sequence can be seen as a series of body skeletons with different joint positions at each time step. Let $S_{xyz} \in \mathbb{R}^{N \times M \times 3}$ be the matrix representation of such a sequence of body skeletons with $N$ joints. Each column-vector of the matrix represents one such skeleton with the XYZ joint position coordinates in its entries at a frame $m$. Such a representation is shown as follows:
We treat the motion segmentation problem as an image segmentation problem by transforming the motion sequence to the RGB image domain, much in the spirit of \cite{laraba20173d, ke2017new}. 
In most motion capture file formats \cite{meredith2001motion}, the data is represented in a hierarchical manner, where each child joint's position and orientation is dependent on its parent's. This gives its local transform. To obtain the global transform of a given joint, one simply multiplies its parents' local transforms iteratively to the joint's local transform \cite{meredith2001motion} which is known as Forward Kinematics. Local and global coordinate systems are used in a variety of contexts in Computer Graphics \cite{parent2012computer, akenine2018real}. Usually, objects are kept in their local coordinates in the memory. The global transform in the world, is then computed ad-hoc when needed.
% Janis: complex phrasing. I would rephrase to:
%Most motion capture file formats define a single pose based on a hierarchical skeleton \cite{meredith2001motion}. The transformation of an individual joint is defined in a coordinate system local to its parent joint. Forward Kinematics describes the process of iteratively applying these local transformations to get the joint transform in global coordinate system. 
% Janis: I would leave out the rest of the paragraph, as different approaches operate in different coordinate systems and I would neither support the claim nor do I think it is really relevant for this task...

Let $S_{xyz} \in \mathbb{R}^{N \times M \times 3}$ be the matrix representation of a sequence of body skeletons with $N$ joints in the Cartesian coordinate system. Each column-vector of the matrix represents one such Cartesian pose with the XYZ joint position coordinates in its entries at a frame $m$. Such a representation is shown as follows:
\begin{equation*}
S_{xyz} = 
\begin{pmatrix}
[x_1(1), y_1(1), z_1(1)] & \dots &  [x_1(M), y_1(M), z_1(M)] \\
\vdots & \ddots & \vdots \\
[x_N(1), y_N(1), z_N(1)] & \dots &  [x_N(M), y_N(M), z_N(M)] \\
\end{pmatrix}
\label{eq:motion matrix}
\end{equation*}
$N$ and $M$ represent number of joints and frames,  respectively.
The values in $S_{xyz}$ are then normalized to the interval [0, 255]. The maximum value in each X-, Y- and Z-dimension within one motion sequence is set to 255, while the lowest one in each dimension is set to 0. Finally, we scale the resulting images vertically to a fixed height $H$ using bi-cubic interpolation such that our method can be applied to motions with different number of joints and skeletons. For our experiments we set $H = 224$. An example of the resulting RGB \emph{motion image} can be seen in Fig. \ref{fig:motion_image_mixed}.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/walk_001_1_global_seg.png}
    \vspace{1mm}
    \includegraphics[width=\linewidth]{images/walk_001_1_local_seg.png}
    \includegraphics[width=\linewidth]{images/walk_019_3_global_seg.png}
    \includegraphics[width=\linewidth]{images/walk_019_3_local_seg.png}
    \caption{Global and local coordinates of two walking sequences. The first and the third image show the motion images obtained from XYZ coordinates in global space, while the second and fourth images show the motion images obtained from the local XYZ coordinate space. Despite both sequences only containing walking and standing actions, the images obtained from global coordinates look very different from each other, while the ones obtained from local space have a homogeneous pattern. The boundaries of the left and right steps are highlighted. Note how in the motion images obtained from local coordinates each step has the same color pattern, while in the images obtained from global coordinates the colors differ from each other and the step boundaries are not as clearly visible.}
    \label{fig:local_vs_global_coords}
\end{figure}

When applying our method on global and local coordinate systems (Fig. \ref{fig:local_vs_global_coords}), we see that motion images with global coordinates look vastly different from each other, despite showing the same action. Hence, making it harder to detect specific patterns. Thus, we propose a normalization method specifically for motion data by using the local coordinates instead. We obtain them by setting the local transform of the root joint to 0. Motion images from these coordinates look similar to each other for the same type of action. Even a human observer can see some patters in the motion images obtained from local XYZ coordinates as shown in Fig. \ref{fig:local_vs_global_coords}. Using the local coordinates, keeps the RGB values in the same range for the same motions, i.e. a left step looks the same (only translated within an image) across all images. Additionally, a side benefit of using local coordinates as a normalization technique is that in most cases, they are already provided from the source files.

%\textbf{Local Coordinates as Normalization.} For many machine learning algorithms, such as SVM \cite{??}, K-nearest neighbor \cite{??} or neural network classifiers \cite{??}, feature normalization is an important pre-processing step \cite{??}. In image classification, for example, the mean RGB value across all training images is computed and then subtracted from each image that is supposed to be classified \cite{??}. Other forms of normalization are scaling the features, such that the covariance is the same, or Whitening \cite{??}. The latter achieves minimum correlation among all features. LeCun highlighted the importance of these normalization techniques in terms of convergence speed in \cite{??}. However, these techniques are very general in nature and not task specific. Since we know, we only deal with motion capture data, we propose a simpler normalization method based on the nature of motion capture file formats.

%In most motion capture file formats \cite{??}, the data is represented in a hierarchical manner, where each child joint's position and orientation is dependent on its parent's. This gives its local transform. To obtain the global transform of a given joint, one simply multiplies its parents' local transforms iteratively to the joint's local transform \cite{??}. The use of a local coordinate and a global coordinate system is used in a variety of contexts in Computer Graphics \cite{??}. Usually, objects are kept in their local coordinates in the memory. The global transform in the world, is then computed ad-hoc when needed. It is done by first rotating the object in its local coordinates and then translating it, to its global position. This representation in local and global coordinates circumvents problems such as the Gimbal lock \cite{??}. We define $$\vec{\textbf{x}} = \begin{pmatrix}x\\y\\z\end{pmatrix}$$ as the local coordinates of some joint and $$\vec{\textbf{x}}' = \begin{pmatrix}x'\\y'\\z'\end{pmatrix}$$ as its global coordinates. The global coordinates are obtained via $\vec{\textbf{x}}' = A\vec{\textbf{x}}$, where $A$ is a transformation matrix. $A$ can be decomposed into a rotation matrix $R$ and a translation matrix $T$ with $A = RT$. $A$ can be different for each frame, e.g. in a walking action the translation of all joints of the walking character changes, as well as the orientation of some joints. Due to this, different coordinate values for the same motions, such as left step and right step, are obtained. When displaying our motion data as motion images (Fig. \ref{fig:local_vs_global_coords}), we see that motion images with global coordinates look vastly different from each other, despite showing the same action. Hence, making it harder to detect specific patterns. Due to this we propose a normalization method specifically for motion data by using the local coordinates instead. We obtain them by setting the local transform of the root joint to 0. Motion images from these coordinates look similar to each other for the same type of action. Even a human observer can see some patters in the motion images obtained from local XYZ coordinates as shown in Fig. \ref{fig:local_vs_global_coords}. Using the local coordinates, keeps the RGB values in the same range for the same motions, i.e. a left step looks the same (only translated within an image) across all images. Additionally, a side benefit of using local coordinates as a normalization technique is that in most cases, they are already provided from the source files.

==> sections/04_dtfcn.tex <==
\section{Dilated Temporal Fully-Convolutional Networks}
In this section, we describe our network architecture for semantic segmentation of motion images. We refer to the presented architecture as dilated temporal fully-convolutional network (DT-FCN) to emphasize the inspiration behind our model. Before we start defining our network architecture, we highlight the nature of semantic segmentation and sequence modeling tasks for images and time dependent data to discuss similarities and differences between our proposed network and previous models \cite{long2015fully, bai2018empirical} that have tackled similar problems.

\subsection{Semantic Segmentation of Images}
\label{sec:image_segmentation}
Semantic segmentation of images refers to the dense labeling of pixel data, where each pixel value is assigned a distinct label, depending on structural features in spatial neighborhood regions. Such a model produces a mapping of the form $f: X \rightarrow Y$, where $X(i, j) \in \mathbb{R}^{N \times M \times D}$ and $Y(i, j) \in \mathbb{R}^{N \times M \times C}$. $N$ represents the height of the image and $M$ the width. The number of channels is given by $D$, while the number of classes is represented by $C$. For each pixel $(i, j)$ in $Y$, a vector of length $C$ is computed with the probabilities of each class defining that pixel. The final pixel labels are then often given by $c(i, j) = \argmax Y(i, j)$. Such labeling does not only provide a segmented output but each pixel also provides semantic meaning.

\textbf{Fully-Convolutional Neural Networks.} Long et al. \cite{long2015fully} have popularized the idea of using fully-convolutional neural networks (FCN) for semantic segmentation of images. In contrast to traditional CNNs that do not extend to arbitrary-sized inputs, due to the use of fully-connected or dense layers, FCNs \emph{convolutionize} \cite{lin2013network} these layers in CNNs. To overcome coarse predictions, Long et al. propose \emph{skip} connections \cite{long2015fully}, which incorporate features from prior layers in the final output.

\subsection{Sequence Modeling}
In sequence modeling tasks, we are given an input sequence $x_0, x_1, ..., x_{t-1}, x_t$ and want to predict some corresponding output sequence $y_0, y_1, ..., y_{t-1}, y_t$. Usually, this is under the constraint that an output $y_t$ can only be predicted using samples that have been observed before time $t$, i.e. samples at times $0, ..., t-1$. Thus, our mapping function in this case is $f: x(t-A, ..., t-1) \rightarrow y(t)$ with $A \geq 1$ for an output $y$ at a given time step $t$. 
%In recent years, such sequence modeling tasks have been associated with recurrent architectures of neural networks only \cite{Goodfellow, CourseraSequence}. However, recent research \cite{bai2018empirical, wavenet, Lea2017TemporalCN} shows that certain convolution-based neural architectures reach state-of-the-art results in various sequential tasks. Such architectures that deal with sequential, time-dependent data, are called Temporal Convolutional Networks (TCN) \cite{bai2018empirical,Lea2017TemporalCN, lea2016temporal}. To our knowledge, Lea et al. \cite{lea2016temporal} were the first ones to use this term. Later, Bai et al. published an extensive description of the features of such networks in their study \cite{bai2018empirical}. Hence, we will go by their definition of a TCN in this paper.


\textbf{Temporal Convolutional Neural Networks.}
According to \cite{bai2018empirical}, the two distinguishing characteristics of TCNs are:
\begin{enumerate}
\item The architecture can take a sequence of any given length and map it to another sequence of the same length.
\item There is no \emph{leakage} from the future to the past, i.e. the mapping has to be \emph{causal}, such that a future output at time $t$ can only depend on past inputs at times $0, ..., t-1$.
\end{enumerate}
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.6\linewidth]{images/acausal_vs_causal.png}
%    \caption{Acausal (left) and causal (right) convolution. The causal convolution takes inputs from the past to compute the output at time step $t$, while the acausal convolution also takes future inputs into account.}
%    \label{fig:acausal_vs_causal}
%\end{figure}
The first characteristic can be obtained by adding zero padding of length (kernel size - 1) to each layer, so that subsequent layers have the same lengths as previous ones. The second characteristic is ensured by the use of causal convolutions. These convolve an input $X$ at each time step $t$ from $X_{t-w}$ to $X_t$, where $w$ is the length of the filter, while acausal convolutions convolve it from $X_{t-\frac{w}{2}}$ to $X_{t+\frac{w}{2}}$.

\subsection{Semantic Segmentation of Motion Images}
While image segmentation is based on segmenting \emph{spatially} similar regions, the idea of sequence segmentation is to extract structurally similar regions in the same \emph{temporal} neighborhood. Semantic segmentation adds a higher level meaning to each of these segments by adding a semantic label to each region. Hence, semantic segmentation of sequences can be considered a dense labeling of time steps. Since the aim is not to predict future data based on previous observations, the classification is allowed to also consider future samples to derive more accurate labels. Hence, given an input sequence $x_0, x_1, ..., x_t, ..., x_T$ our mapping function can be considered to be $f: x(t-A, ..., t, ..., t+B) \rightarrow y(t)$ for an output $y$ at time $t$ with suitable adjustments at the borders. This allows us to use acausal convolutions in contrast to the previously mentioned TCN architecture. Since our goal is to semantically segment motion images, the mapping function is further extended in its input: $f: X \rightarrow y(0, ..., T)$, where $X$ is now a matrix of the dimensions $\mathbb{R}^{N \times M \times 3}$, similar to the mapping in image segmentation tasks (Section \ref{sec:image_segmentation}). Due to the allowance of leakage from the future in this segmentation task, we propose an acausal architecture, similar to previous FCN models, with the difference that it filters the input in the temporal dimension only (akin to previous TCN architectures). To ensure dense labeling and an output of the same length as the input, we also zero-pad each hidden layer, as in \cite{bai2018empirical}. This makes our model simpler compared to Long et al. \cite{long2015fully} because we do not need to make use of skip connections.

\subsection{Temporal 2D Convolution}
Our data consists of three-dimensional motion images, where one dimension represents the time, the other the spatial properties and relations of the joints to each other and the third the 3D joint positions. Since we only want to segment it along the time dimension, we use a 2D convolution in which the connections are local in the time dimension only but full along the other dimensions:
\begin{align}
S \star K = \vec c(i) = \sum_{n=0}^{N-1}\sum_{m=0}^{M-1}\sum_{d=0}^{2} S(n, m, d) \cdot K(n, i-m, d)
\end{align}
Where $S$ is the input motion image in $\mathbb{R}^{N \times M \times 3}$ and $K$ the filter kernel in $\mathbb{R}^{N \times w \times 3}$, where $w$ is the filter width. To map this to common deep neural network frameworks \cite{chollet2015keras, tensorflow, jia2014caffe}, we use a filter height, which is equal to the input image height. The filter width and stride in the time dimension can be chosen arbitrarily. Such a convolution is depicted in Fig. \ref{fig:2d_conv_tmp}. To keep the output length the same as the input, we add a two-dimensional zero-padding of size $N \times \lfloor \frac{w}{2} \rfloor$ on each side of the temporal dimension.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{images/2D_temp_conv.png}
    \caption{A two-dimensional acausal temporal convolution can be achieved by setting the filter height equal to the input height.}
    \label{fig:2d_conv_tmp}
\end{figure}

\subsection{Dilated Convolutions}
\label{sec:dilated_conv}
Since motion features can span many frames, the filter needs to be able to look far into the future and into the past. For example, when distinguishing between labels like \emph{left step} (step while walking) from \emph{begin} and \emph{end left step} (step from/to standing position), there are often many time steps between the beginning and ending of a full step. Thus, our network needs a large receptive field. A normal CNN is only able to look at a window linear to the depth of the network. This requires many layers and parameters to train. Following the work of van den Oord et al. \cite{wavenet}, we apply dilated convolutions (also known as \emph{\'a trous} or convolution with holes \cite{holschneider1990real}) that enable exceptionally large receptive field sizes \cite{yu2015multi}. Such a convolution filter is essentially the equivalent to a larger filter, which has been derived from the original filter, dilated with zeros, but is significantly more efficient. The dilation allows the filter to operate on a coarser scale than a normal convolution. For 1D sequence $\textbf{x} \in \mathbb{R}^N$ and filter $f: \{0, ..., k-1\} \rightarrow \mathbb{R}$ such a convolution is formally defined as:
\begin{equation}
(\textbf{x} *_d f)(t) = \sum_{i=0}^{k-1} f(i) \cdot \textbf{x}_{s-d \cdot i}
\end{equation}
where $d$ is the dilation and $k$ the filter length. A normal convolution thus can be seen as a special case of a dilated convolution with $d=1$. Fig. \ref{fig:dilation} shows how systematic dilation increases the receptive field size exponentially in depth with comparably few layers and parameters. A receptive field size of 15 time steps is already obtained after three layers using a filter width of three. For a non dilated convolution with the same width, we would need seven layers and more than double the parameters to achieve the same receptive field size (see Fig. \ref{fig:dilation}).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/dilation_EG.png}
    \caption{Dilated (left) and undilated (right) convolution. Systematic dilation increases the receptive field size exponentially with depth, with considerably fewer layers and thus parameters to be trained.}
    \label{fig:dilation}
\end{figure}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{images/dtfcn.png}
    \caption{Our dilated temporal fully-convolutional neural network (DT-FCN) for motion capture segmentation. The initial layer consists of a traditional 2D convolutional layer, applied in the time dimension. The next layers are 1D temporal acausal convolutions with dilation. The final layer is a convolutionized dense-layer with a Softmax activation function.}
    \label{fig:dtfcn}
\end{figure*}

\subsection{Network Architecture}
\label{sec:architecture}
%In this section we describe our complete network architecture in more detail. We first begin with the biological inspiration of our model and then describe more technical details.
%Our visual system consists of a hierarchy of multiple subsequent processing stages in which the nature of the visual features becomes systematically more abstract, invariant, and general \cite{blasdel1984physiological, cheema2016optimum}. As an example, our entire ventral stream consists of five visual cortex areas (V1 - V5) \cite{Remington2012233, blasdel1984physiological} of which each becomes more abstract and complex with each hierarchy level. The nature of such an architecture of having five major visual processing stages, has been adapted to many convolutional neural network architectures, such as AlexNet \cite{krizhevsky2012}, CaffeNet \cite{jia2014caffe} or the VGG networks \cite{VGG}. In fact, when such neural architectures are trained on a general set of images, Gabor-like V1 filters form in the early layers of these networks \cite{krizhevsky2012}, which have been associated with our primary visual cortex (V1 area). More complex filters are formed in higher hierarchy levels, similar to the higher hierarchical levels in our visual pathway. This is akin to the five areas in our visual cortex. 
Inspired by the five major visual cortex areas (V1 - V5) \cite{Remington2012233, blasdel1984physiological} in the human visual system, our model has a total of five convolution layers. To process three-dimensional image data, the initial one consists of an acausal temporal 2D convolution, followed by four subsequent layers of 1D temporal dilated acausal convolutions. An overview of our architecture can be seen in Fig. \ref{fig:dtfcn}. Each of these five conv-layers uses a ReLU \cite{krizhevsky2012} non-linearity as activation function. Similar to \cite{VGG, he2016deep}, we use the same width $w$ for each convolution layer with a stride of 1. To make sure that an output of the network's receptive field depends on every input within that receptive field, the dilation rate $d$ increases with each layer $l$ according to $d = w^{l-1}$. After these a dropout of 50\% is used in the training to counter over-fitting and a final convolutionized dense-layer \cite{lin2013network, long2015fully} with a Softmax \cite{sutton1998reinforcement} activation function is added after that. To ensure that the values created by the ReLU activation layers before the Softmax function, do not exceed reasonable input values, we normalize the output of the last ReLU activation using the following function:
\begin{align}
NormReLU(x) = \frac{ReLU(x)}{\max(ReLU(x)) + \epsilon}
\end{align}
We use a value of $\epsilon = 1e^{-5}$ and found that this greatly improves accuracy. Finally, we upsample the output to the full image height for visualization purposes.

%We then pass it to our network (Fig. \ref{fig:dtfcn}). Akin to the five areas in our visual cortex, our model has a total of five convolution layers. The initial layer consists of a traditional 2D convolutional layer with a kernel height of the image, which is only applied in the time dimension. The next four layers are 1D temporal acausal convolutions with dilation. Every layer has the same convolution width $w$ with stride 1. The dilation rate $d$ increases with each layer $l$, according to $d = w^{l-1}$. The number of channels increases with each layer by a factor of two, until it reaches 512. A convolutionized dense layer is added after that. To reduce oversegmentation we add a max-pooling layer and upsample the output.

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{images/model}
% \caption{Overview of our model. The motion capture sequence is transferred to an RGB-domain and, together with its semantic labels, fed to the network as input. The output is a semantic classification of each motion frame.}
% \label{fig:model}
% \end{figure}

% \begin{figure*}
% \centering
% \includegraphics[width=0.92\linewidth]{images/tfcn_janis}
% \caption{Our dilated temporal fully-convolutional neural network (DTFCN) for motion capture segmentation. The initial layer consists of a traditional 2D convolutional layer. The next layers are 1D temporal acausal convolutions with dilation. To reduce oversegmentation we add a final max-pooling layer and upsample the output. We use a total of five convolution layers, of which four are temporal dilated layers.}
% \label{fig:tfcn}
% \end{figure*}

==> sections/05_evaluation.tex <==
\section{Evaluation}
%This section describes various experiments and tests carried out to evaluate the performance of the presented motion capture segmentation approach. We compare our model against a popular RNN method for sequence modeling \cite{lstm} and two state-of-the-art TCN-based action segmentation models \cite{lea2016temporal, Lea2017TemporalCN}. We evaluate them on the described data set in Section \ref{sec:dataset}.
%Erik
This section describes experiments carried out to evaluate the performance of the presented motion capture segmentation approach. The implementation details are given in Section \ref{sec:impl_details} and the data set is described in Section \ref{sec:dataset}. We evaluate the robustness of the presented approach under noise levels in Section \ref{sec:noise}. The effect of the receptive field size of our model on the accuracy of the predictions is demonstrated in Section \ref{sec:recep}. Finally, in Section \ref{sec:benchmark} we compare our method against a popular RNN method for sequence modeling \cite{graves2005framewise} and two state-of-the-art TCN-based action segmentation models \cite{lea2016temporal, Lea2017TemporalCN}. 


\subsection{Implementation Details}
\label{sec:impl_details}
%Our model's parameters are learned using the categorical cross entropy loss with Stochastic Gradient Descent and the Adam optimizer \cite{kingma2014adam}. We use the default settings of $\alpha = 0.001, \beta_1 = 0.9, \beta_2 = 0.999$ and $\epsilon=10^{-8}$ as described in the paper. For implementation we use Keras \cite{chollet2015keras} with a Tensorflow \cite{tensorflow} back-end. In all of our experiments, we use non-randomized 7-fold cross-validation and 100 training epochs.
%Erik
Our model's parameters are learned using the categorical cross entropy loss with Stochastic Gradient Descent and the Adam optimizer \cite{kingma2014adam}. We use the default settings of $\alpha = 0.001, \beta_1 = 0.9, \beta_2 = 0.999$ and $\epsilon=10^{-8}$. We implemented the network using Keras \cite{chollet2015keras} with a Tensorflow \cite{tensorflow} back-end. In all of our experiments, we use non-randomized 7-fold cross-validation and 100 training epochs.

\subsection{Data Set}
\label{sec:dataset}
Our motion capture data set consists of 70 sequences in total, of which 60 are used for training and 10 for testing. The data set contains standing, walking, picking, placing, and turning actions. For supervised training these have been segmented and labeled into the following 10 motion primitives by hand:

\begin{table}[h]
    \centering
    \begin{tabular}{l|c|c}
       Motion Primitive & Description & Color \\
       \hline
       standing & standing in T or ``normal" pose& \ColorSquare{none} \\
       begin left step  & left step from a standing pose & \ColorSquare{beginLeftStep} \\
       begin right step & right step from a standing pose & \ColorSquare{beginRightStep} \\
       left step & left step within locomotion & \ColorSquare{leftStep} \\
       right step & right step within locomotion & \ColorSquare{rightStep} \\
       end left step & left step to a standing pose & \ColorSquare{endLeftStep} \\
       end right step & right step to a standing pose & \ColorSquare{endRightStep} \\
       reach & reach out with arm & \ColorSquare{reach} \\
       retrieve & retrieve with arm & \ColorSquare{retrieve}\\
       turn (while standing) & turn body in different direction & \ColorSquare{turnRight}\\
    \end{tabular}
    \caption{Motion primitive labels with their corresponding label color in the segmented images.}
    \label{tab:dataset}
\end{table}

\subsection{Evaluation of Robustness}
\label{sec:noise}
\textbf{Random Noise Injection.} To test the robustness of the evaluated models against noisy training labels we gradually add noise to the training labels. We do this by setting a certain percentage of frames within one motion sequence to a random label of the given 10 labels (Fig. \ref{fig:noise_labels}). We add noise in 10\% intervals. We start from 0\% noise and gradually increase the noise level by additional 10\% until we reach 100\%.
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/noise_labels}
\caption{Training labels of a sample training sequence with random noise injection. Percentage of noise from top to bottom: 0\%, 10\%, 20\%, 30\%, 40\%, 50\%, 60\%, 70\%, 80\%, 90\%, 100\%}
\label{fig:noise_labels}
\end{figure}
%While training a network on 100\% noise will not tell us anything about its robustness, we use this test as a ``reality-check'' to make sure that there is no bug in our code. The accuracy for this experiment should be around $\sim$10\% across all models, since randomly picking the right label from 10 given labels is 10\%.
%Erik
We use 100\% noise as ground truth with an expected accuracy of $\sim$10\% across all models.

 \textbf{Noisy Boundary Regions.} While the data set with random noise injection gives us some evaluation form for robustness against noise, it is not very applicable for ``real-world noise" in training labels. In reality, annotation disagreements usually happen around segment boundaries. Bouchard et al. \cite{bouchard2007semantic} have shown that a single person determines the segmentation boundaries within the same sequence differently every time they segment it. The median of each segment boundary was computed and then the distance of each boundary from the median was computed and graphed as a histogram. The result is a standard deviation of 15.4 frames, or about $\frac{1}{2}$ seconds. Due to these inter- and intra-annotator disagreements, we adapt our initial data set (without any noise) and insert wrong information, i.e. noise, in a window around a segment boundary frame (Fig. \ref{fig:noise_windows}). A boundary frame is determined by using the first frame of a new segment within a sequence. The width of the noise windows is set to $w_{noise} = 2n + 1$. Within this window we set the frames to a random label. We chose $n = \{5, 10, 15\}$ frames. The resulting training sequence labels are illustrated in Fig. \ref{fig:trans_noise}.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth, height=0.5cm]{images/noise_windows}
\caption{Boundary noise windows (highlighted with green edges). The line between two segments indicates a boundary frame. Frames within the green windows are set to random labels.}
\label{fig:noise_windows}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth, height=1.7cm]{images/trans_noise}
\caption{Boundary noise labels for an example training sequence. From top to bottom: $w_{noise} = 11$ frames, $w_{noise} = 21$ frames, $w_{noise} = 31$ frames, original sequence segmentation.}
\label{fig:trans_noise}
\end{figure}

\subsection{Evaluation of Receptive Field Size}
\label{sec:recep}
In order to determine the optimal receptive field size (RFS) for our model, we test our described architecture on different convolution kernel widths $w$. For this we choose a model that just uses a single frame for its evaluation ($w = 1$, RFS = 1 frames), one that has a RFS of local structures in a sequence ($w = 3$, RFS = 243 frames, see Fig. \ref{fig:recep243}) and one that is bigger than the longest sequence in our dataset ($w = 5$, RFS = 3125 frames). Table \ref{tab:rfs-models} shows the different RFS after each layer for the three versions that we evaluate of the architecture described in section \ref{sec:architecture}. The receptive field size $\text{RFS}_L$ after each layer $L$ is calculated by 
\begin{align}
\text{RFS}_L = 1 + \sum_l^L (w_l - 1) \cdot d_l
\end{align}
where $d_l$ is the dilation rate and $w_l$ the convolution kernel width at layer $l$.

\begin{table}[h]
\centering
\label{tab:rfs-models}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|}
\cline{2-10}
& \multicolumn{3}{|c|}{$w = 1$} & \multicolumn{3}{|c|}{$w = 3$} & \multicolumn{3}{|c|}{$w = 5$}\\
\hline
\hline
\multicolumn{1}{|c|}{$L$} & $d$ & $p$ & RFS & $d$ & $p$ & RFS & $d$ & $p$ & RFS\\
\hline
\hline
\multicolumn{1}{|c|}{1} & 1 & 1 & 1 & 1 & 2 & 3 & 1 & 4 & 5 \\
\hline
\multicolumn{1}{|c|}{2} & 1 & 1 & 1 & 3 & 6 & 9 & 5 & 20 & 25 \\
\hline
\multicolumn{1}{|c|}{3} & 1 & 1 & 1 & 9 & 18 & 27 & 25 & 100 & 125 \\
\hline
\multicolumn{1}{|c|}{4} & 1 & 1 & 1 & 27 & 54 & 81 & 125 & 500 & 625 \\
\hline
\multicolumn{1}{|c|}{5} & 1 & 1 & 1 & 81 & 162 & 243 & 625 & 2500 & 3125 \\
\hline
\multicolumn{1}{|c|}{\#$P$} & \multicolumn{3}{|c|}{225,290} & \multicolumn{3}{|c|}{663,562} & \multicolumn{3}{|c|}{1,101,834}\\
\hline
\end{tabular}
\caption{Model architectures and their receptive field sizes (RFS) in frames after each layer $L$ for our proposed architecture. $w$ is the kernel width, $d$ the dilation rate and $p$ the padding. \#$P$ describes the number of parameters in each model.}
\end{table}

\begin{figure}[h]
\includegraphics[width=\linewidth]{images/recep_243}
\caption{Receptive field size of 243 frames highlighted on a 1193 frame sequence.}
\label{fig:recep243}
\end{figure}

We evaluate these three models on our data set described in section \ref{sec:dataset} with random noise injection. Fig. \ref{fig:noise} shows  that even though a width $w = 5$ (RFS: 3125 frames) covers the entire sequence, the test accuracy is worse on all noise levels compared to using $w = 3$ (RFS: 243 frames). This is in contrast to popular claims \cite{bai2018empirical, wavenet} in sequence modeling tasks that the receptive field of the network should at least cover the longest sequence in the data set. It supports a more intuitive suggestion that local structures (e.g. in Fig. \ref{fig:recep243}) are enough to be able to classify important structural and temporal information. Furthermore, the increase in parameter space for $w = 5$ make it also more prone for over-fitting, as compared to $w = 3$.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/noisy_exp}
\caption{Test accuracies for different receptive field sizes of our proposed architecture depending on noise level. The model with RFS = 243 (\emph{red}) constantly outperforms the others. Note how at 80\% of noise in training labels still an accuracy of almost 90\% in the test set is achieved. \emph{Red}: RFS = 243, \emph{black}: RFS = 3125, \emph{blue}: RFS = 1.}
\label{fig:noise}
\end{figure}

\subsection{Evaluation Against Benchmark Models}
\label{sec:benchmark}

We compare the accuracy of our model against three state-of-the-art methods: Firstly, a bidirectional LSTM (Bi-LSTM) model \cite{graves2005framewise}, which is a widely used architecture for sequence modeling tasks and can theoretically have an infinite ``receptive field size''\cite{ zeyer2017comprehensive}. Secondly, an acausal encoder-decoder TCN model (ED-TCN) proposed by Lea et al. \cite{lea2016temporal, Lea2017TemporalCN}. Finally, we compare our method against a causal TCN architecture with dilated convolutions (DilatedTCN), which was adapted by Lea et al. \cite{Lea2017TemporalCN} from the original WaveNet architecture \cite{wavenet}.

While evaluating the benchmarks against our best model ($w = 3$), we found that they performed significantly worse when the input values are between [0, 255]. Hence, we adjust the input values for the benchmark models according to their activation functions by scaling them between [-1, 1] for a fairer comparison, while keeping them between [0, 255] for our proposed models. 

%The following three benchmarks are used for comparison:

%\textbf{Bidirectional LSTM.} LSTMs are a widely used method in sequence modeling tasks \cite{??}. They have been the go-to method for sequential data and have been successfully used in action segmentation tasks \cite{??}. For these experiments we use a more sophisticated LSTM architecture which is also able to take information from future samples, called a bidirectional LSTM \cite{lstm}. Fig. \ref{??} illustrates the model. LSTM's can theoretically have an infinite ``receptive field size''.

%TODO: insert figure

%\textbf{Encoder-Decoder TCN.} The next model we compare against is also an acausal TCN method, similar to ours. However, it has an encoder-decoder nature to it. It is proposed by Lea et al. \cite{lea2016temporal, Lea2017TemporalCN} as a state-of-art action segmentation method in videos. We adapt their network for motion image segmentation. Fig. \ref{??} shows an overview of their Encoder-Decoder TCN. First the input is filtered using a convolutional layer and then subsampled with a max-pooling layer to obtain the most important information. This is repeated until the decoding layers are reached. The decoding layers reverse the process by upsampling the subsampled features and performing a convolution on the upsampled output. Lea et al. use two encoding and two decoding layers with convolution kernels of width $w = 25$ each time. Each having a convolution and the respective upsampling or downsampling operation. The total receptive field size is 49 frames for the entire network.

%TODO: insert figure

%\textbf{DilatedTCN (WaveNet adaptation.)} DilatedTCN is an adaptation by Lea et al. \cite{Lea2017TemporalCN} from the original WaveNet architecture proposed by van den Oord et al. \cite{wavenet} for audio synthesis. They adapt it for the task of action segmentation. While they conduct experiments on an causal and acausal architecture, we stick in our experiments to the originally proposed causal WaveNet model to see how causality effects segmentation behavior. Nevertheless, we use the hyper-parameters suggested by Lea et al. Their WaveNet adaption is illustrated in Fig. \ref{??}. Each of the one-dimensional convolution layers has a dilation rate of $d=2^l$ within one block. Furthermore, residual connections are applied between each convolution layer. Every block of three convolutions is then connected with skip connections which essentially merge the feature-maps together by summing them up \cite{??}. Lea et al. use 1 block with 4 layers and 3 blocks with 6 layers each. Their total receptive field is 254 frames.

%TODO: insert figure

\textbf{Vanilla Labels Experiment.} We first test our best model ($w =3$) and the benchmark models on the ``vanilla" labels without any noise and then gradually increase the noise levels by 10\% as described in section \ref{sec:dataset} in \emph{Random Noise Injection}. Fig. \ref{fig:results00} shows the segmentation results for the benchmark models and our best model on a sample test sequence without any noise added into the training data. While DilatedTCN and ED-TCN have similar training and test accuracies (Tab. \ref{tab:results}), the segmentation results of DilatedTCN tend to suffer more from over-segmentation, especially at the boundary frames. Bi-LSTM suffers the most from such an over-segmentation. Our model achieves similar results to ED-TCN, when trained on a clean data set (Fig. \ref{fig:results00} bottom row). However, it makes use of less than half of the parameters, while achieving better results in per-frame accuracy (Tab. \ref{tab:results}).

\begin{figure}[h]
\includegraphics[width=\linewidth]{images/Results_0}
\caption{Segmentation results of benchmark models, as well as our best model ($w = 3$) on an example test sequence. The top half of each row is the ground truth segmentation of the depicted motion image, while the bottom half is the prediction from the respective network. Results show ``typical'' performance of each model across data set. Training was done without any noise added to the labels.}
\label{fig:results00}
\end{figure}

\begin{table}[h]
\centering
\begin{tabular}{ |l|c|c|c|c| }
  \hline
  & Bi-LSTM & ED-TCN & DilatedTCN & Ours\\
   & \cite{graves2005framewise} & \cite{lea2016temporal} & \cite{Lea2017TemporalCN} & ($w = 3$)\\
  \hline
  Train & 86.32\% & 90.05\% & 90.64\% & \textbf{95.42\%}\\
  Test & 81.95\% & 88.69\% & 88.47\% & \textbf{90.81\%}\\
  \hline
  \# Param. & 378,634 & 1,613,770 & 388,874 & 663,562\\
  \hline
  RFS & $\infty$ & 49 & 254 & 243\\
  \hline
  Causality & Acausal & Acausal & Causal & Acausal\\
  \hline
\end{tabular}
\caption{Per-frame accuracy for benchmark models and our best model ($w = 3$) on the data set without any noise in the training labels.}
\label{tab:results}
\end{table}

\textbf{Random Noise Injection Experiment.} Gradually adding noise to the training data reveals that up until 60\% added noise, all networks perform similar to their performance at 0\% noise, as shown in Tab. \ref{tab:noise_results}. However, beyond that the performance of DilatedTCN already starts to deteriorate. ED-TCN stays robust up until 70\% of added noise, while the per-frame accuracy of Bi-LSTM and our model stays on a steady level up until 80\% noise. However, in contrast to Bi-LSTM our model consistently outperforms all other benchmarks on every noise level, while Bi-LSTM performs the weakest at noise levels lower than 80\%. The results in Tab. \ref{tab:noise_results} show that a mere 10\% of correct information is needed for our model to perform as well as Bi-LSTM at a 0\% noise level. Furthermore, 20\% of information is enough to achieve usable segmentation results, which is further backed by our segmentation results shown in Fig. \ref{fig:our_noisy_pred}. Fig. \ref{fig:noise_bench_80} and \ref{fig:noise_bench_90} show a sample prediction of the tested models at 80\% and 90\% training label noise, respectively. DilatedTCN averages the output to the background class when 90\% of noise in the training labels is used, while the others still obtain reasonable segmentation results. Our model struggles with over-segmentation more than the other models at 90\% noise.

\begin{table}[h]
\centering
\begin{tabular}{ |c|c|c|c|c| }
  \hline
  Noise in & Bi-LSTM & ED-TCN & DilatedTCN & Ours\\
   Training & \cite{graves2005framewise} & \cite{lea2016temporal} & \cite{Lea2017TemporalCN} & ($w = 3$)\\
  \hline
  0\% & 81.95\% & 88.69\% & 88.47\% & \textbf{90.81\%}\\
  10\% & 83.70\% & 89.16\% & 89.37\% & \textbf{90.99\%}\\
  20\% & 79.94\% & 89.46\% & 88.86\% & \textbf{90.75\%}\\
  30\% & 85.02\% & 89.40\% & 88.90\% & \textbf{91.20\%}\\
  40\% & 84.29\% & 89.02\% & 88.64\% & \textbf{91.13\%}\\
  50\% & 81.72\% & 87.40\% & 87.93\% & \textbf{91.04\%}\\
  60\% & 83.08\% & 88.65\% & 86.14\% & \textbf{92.99\%}\\
  70\% & 82.16\% & 87.66\% & 79.46\% & \textbf{90.11\%}\\
  80\% & 81.91\% & 80.46\% & 61.82\% & \textbf{89.55\%}\\
  90\% & 71.74\% & 54.91\% & 34.99\% & \textbf{81.18\%}\\
  100\% & 8.76\% & 10.39\% & 11.85\% & 11.24\%\\
  \hline
\end{tabular}
\caption{Per-frame test accuracy for benchmark models and our best model ($w = 3$) with noise added into the training labels.}
\label{tab:noise_results}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth, height=6cm]{images/our_noisy_prediction}
\caption{Segmentation results of an example training sequence of our $w = 3$ model. The noisy labels it has been trained on are on top of its respective predictions. The first result shows the result for 0\% noise, while the last for 100\%. Noise is added in +10\% intervals.}
\label{fig:our_noisy_pred}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/noise_exp_80_modified}
\caption{Segmentation results for training on 80\% label noise. Bottom row shows the actual segmentation label without any noise for comparison. Example shows ``typical'' performance of networks across the dataset.}
\label{fig:noise_bench_80}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/noise_exp_90_modified}
\caption{Segmentation results for training on 90\% label noise. Bottom row shows the actual segmentation label without any noise for comparison. Example shows ``typical'' performance of networks across the data set.}
\label{fig:noise_bench_90}
\end{figure}

\textbf{Boundary Noise Experiment.} Since human annotators usually disagree the most in the boundary regions between two adjacent segments, we conduct an experiment where a window of width $w_{noise}$ at a boundary frame contains randomly set, and hence wrong, training labels, as described in Section \ref{sec:dataset} \emph{Noisy Boundary Regions}. 
Table \ref{tab:trans_noise_results} shows that despite DilatedTCN having the worst robustness performance in the previous noise experiment, it overall performs second best in terms of per-frame accuracy with $w_{noise} = \{21, 31\}$. 
Our network architecture still outperforms the other benchmark models, however. Fig. \ref{fig:trans_noise_results} shows an example training sequence, as well as the predicted segmentation by our model ($w = 3$) and benchmarks for $w_{noise} = \{11, 21, 31\}$. While the boundary prediction is almost perfect for $w_{noise} = 11$ in all models except DilatedTCN, one can see visible artifacts in the boundary regions with a noise window width of $w_{noise} = 21$ and $w_{noise} = 31$. Fig. \ref{fig:trans_noise_results} shows that our model consistently performs better than the benchmarks.

\begin{table}[h]
\centering
\begin{tabular}{ |c|c|c|c| }
  \hline
  $w_{noise}$ & 11 frames & 21 frames & 31 frames\\
  \hline
  Bi-LSTM \cite{lstm} & 84.57\% & 81.47\% & 78.94\%\\
  ED-TCN \cite{lea2016temporal} & 88.15\% & 83.82\% & 75.75\%\\
  DilatedTCN \cite{Lea2017TemporalCN} & 87.50\% & 85.48\% & 80.62\%\\
  Ours ($w = 3$) & \textbf{91.45\%} & \textbf{89.03\%} & \textbf{83.59\%}\\
  \hline
\end{tabular}
\caption{Per-frame test accuracies for benchmark models and our best model ($w = 3$). Models were trained on noisy labels with random labels in the boundary regions and tested on non-noisy labels. The boundary noise window width in frames is indicated by $w_{noise}$.}
\label{tab:trans_noise_results}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/trans_noise_results}
\caption{Predicted segmentations by different models. Blocks from top to bottom: $w_{noise} = 11$ frames, $w_{noise} = 21$ frames, $w_{noise} = 31$ frames, original sequence segmentation. our model ($w = 3$) achieves qualitatively superior segmentation results compared to the other models}
\label{fig:trans_noise_results}
\end{figure}

%\textbf{No Boundary Information.} While the results in the \emph{Boundary Noise Experiment} have shown that even when wrong information is given in the boundary regions an accurate boundary computation can still be achieved when the noise window width is not too large, we now want to conduct an experiment, which is less ``harsh'' in nature: Instead of giving wrong information in the transition regions, we give no information to the networks. Essentially, leaving them to their own interpretation of what to make of the frames within the transition windows. We do this by setting the loss within the boundary regions to zero. Hence, the networks should not care if the boundary regions contain noise or even correct information.
\textbf{No Boundary Information.} The results in the \emph{Boundary Noise Experiment} have shown that an accurate boundary computation can still be achieved when wrong information is given in the boundary regions, as long as the noise window width is not too large. Additionally, we conduct an experiment, which is less ``harsh'' in nature: Instead of giving wrong information in the transition regions, we give no information to the networks. Essentially, leaving them to their own interpretation of what to make of the frames within the transition windows. We do this by setting the loss within the boundary regions to zero. Hence, the networks should not be affected by the information in the boundary regions. 

Tab. \ref{tab:no_trans_inf} and Fig. \ref{fig:no_trans_inf_res} show that the accuracy increases for all convolution based models but decreases for the RNN based model, compared to the previous experiment with noise in the boundary regions during training time. Interestingly, some of the per-frame accuracy results are better than the results on the original vanilla labels from Tab. \ref{tab:no_trans_inf_vanilla}. This might be due to inter- and intra-annotator disagreements \cite{bouchard2008automated} as described in Section \ref{sec:noise}. When there is no information given in these regions, the networks may be able to learn some representation from the geometric information itself only. This might be on average more accurate on unseen examples than learning from ``human generated'' annotations, which tend to be different from annotator to annotator (or even from using the same annotator) in boundary regions. Fig. \ref{fig:trans_noise_vs_no_inf} compares the results from Fig. \ref{fig:trans_noise_results} to predictions where the boundary regions are masked out. The third row in each segmentation block corresponds to the latter prediction method. While masking these regions still leaves us with wrong classifications in some cases, the overall accuracy improves. 

\begin{table}[h]
\centering
\begin{tabular}{ |c|c|c|c| }
  \hline
  $w_{noise}$ & 11 frames & 21 frames & 31 frames\\
  \hline
  Bi-LSTM \cite{lstm} & 81.02\% & 80.05\% & 76.71\%\\
  ED-TCN \cite{lea2016temporal} & 88.25\% & 85.88\% & 84.88\%\\
  DilatedTCN \cite{Lea2017TemporalCN} & 89.04\% & 86.80\% & 86.01\%\\
  Ours ($w = 3$) & \textbf{92.42\%} & \textbf{91.93\%} & \textbf{90.48\%}\\
  \hline
\end{tabular}
\caption{Per-frame test accuracies for our model ($w = 3$) and the benchmark models with the masked the boundary regions.}
\label{tab:no_trans_inf}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{ |l|c|c|c|c| }
  \hline
  & Bi-LSTM & ED-TCN & DilatedTCN & Ours\\
   & \cite{lstm} & \cite{lea2016temporal} & \cite{Lea2017TemporalCN} & ($w = 3$)\\
  \hline
  Vanilla & \textbf{81.95\%} & \textbf{88.69\%} & 88.47\% & 91.65\%\\
  11 frames & 81.02\% & 88.25\% & \textbf{89.04\%} & \textbf{92.42\%}\\
  21 frames & 80.05\% & 85.88\% & 86.80\% & 91.93\%\\
  31 frames & 76.71\% & 84.88\% & 86.01\% & 90.48\%\\
  \hline
\end{tabular}
\caption{Per-frame test accuracies for our model ($w = 3$) and the benchmark models with the masked the boundary regions, compared with the results of the \emph{Vanilla Labels Experiment}.}
\label{tab:no_trans_inf_vanilla}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/trans_noise_vs_no_inf}
\caption{Predicted segmentations by our model ($w = 3$). Blocks from top to bottom: $w_{transition} = 11$ frames, $w_{transition} = 21$ frames, $w_{transition} = 31$ frames, original sequence segmentation. Each block consists of the (noisy) training label (top part in block), the corresponding predicted segmentation without masking out the noise (middle part in block) and with masking it out (bottom part of block).}
\label{fig:trans_noise_vs_no_inf}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/trans_noise_no_inf_results.png}
\caption{Predicted segmentations by our ($w = 3$) and benchmark models for no information in transition regions. Blocks from top to bottom: $w_{transition} = 11$ frames, $w_{transition} = 21$ frames, $w_{transition} = 31$ frames, original sequence segmentation.}
\label{fig:no_trans_inf_res}
\end{figure}

To see what our network is seeing when all information, no information and wrong information is given in the boundary regions, we plot the class activation maps (CAMs) \cite{Zhou_2016_CVPR_CAMs} (Fig. \ref{fig:cam11}, \ref{fig:cam21} and \ref{fig:cam31}). As expected the network trained on the noisy boundary regions has more uncertainty across the different class labels. The segment boundaries in some of the shown heatmaps (e.g. for the \emph{standing} class) have transitions which are not as distinct as the ones without noise or even without any information given at all. Interestingly, the transitions are much more distinct when there is no information given in the boundary regions during training time than when the true class labels are given. This is true across all $w_{noise}$ sizes, as well as, almost all CAMs. Again, this might be because the annotations given by humans tend to be more ambiguous in nature due to the inter- and intra-annotator differences. When no information at the boundaries is given, the network is able to detect boundaries using distinctive features in the motion images which are less ambiguous across the data set than the variations obtained by human annotators.

\begin{figure*}[ph!]
\centering
\includegraphics[width=\textwidth, height=\textheight,keepaspectratio]{images/CAM_11}
\caption{Class Activation Maps (CAM) for a boundary window size $w_{noise} = 11$ with an example training sample. From \emph{left} to \emph{right}: CAM without any noise in boundary window for training labels. CAM with no information in boundary window for training labels. CAM with noise in boundary window for training labels. The first row in each column shows the true labels without any noise and the row below that the prediction done by the network when trained on the noisy example. \emph{Top} to \emph{bottom} activation map: \emph{standing} (\ColorSquare{none}), \emph{begin right step} (\ColorSquare{beginRightStep}), \emph{begin left step} (\ColorSquare{beginLeftStep}), \emph{right step} (\ColorSquare{rightStep}), \emph{left step} (\ColorSquare{leftStep}), \emph{end right step} (\ColorSquare{endRightStep}), \emph{end left step} (\ColorSquare{endLeftStep}), \emph{turn} (\ColorSquare{turnRight}), \emph{reach} (\ColorSquare{reach}) and \emph{retrieve} (\ColorSquare{retrieve})}
\label{fig:cam11}
\end{figure*}

\begin{figure*}[ph!]
\centering
\includegraphics[width=\textwidth, height=\textheight,keepaspectratio]{images/CAM_21}
\caption{Class Activation Maps (CAM) for a boundary window size $w_{noise} = 21$ with an example training sample. From \emph{left} to \emph{right}: CAM without any noise in boundary window for training labels. CAM with no information in boundary window for training labels. CAM with noise in boundary window for training labels. The first row in each column shows the true labels without any noise and the row below that the prediction done by the network when trained on the noisy example. \emph{Top} to \emph{bottom} activation map: \emph{standing} (\ColorSquare{none}), \emph{begin right step} (\ColorSquare{beginRightStep}), \emph{begin left step} (\ColorSquare{beginLeftStep}), \emph{right step} (\ColorSquare{rightStep}), \emph{left step} (\ColorSquare{leftStep}), \emph{end right step} (\ColorSquare{endRightStep}), \emph{end left step} (\ColorSquare{endLeftStep}), \emph{turn} (\ColorSquare{turnRight}), \emph{reach} (\ColorSquare{reach}) and \emph{retrieve} (\ColorSquare{retrieve})}
\label{fig:cam21}
\end{figure*}

\begin{figure*}[ph!]
\centering
\includegraphics[width=\textwidth, height=\textheight,keepaspectratio]{images/CAM_31}
\caption{Class Activation Maps (CAM) for a boundary window size $w_{noise} = 31$ with an example training sample. From \emph{left} to \emph{right}: CAM without any noise in boundary window for training labels. CAM with no information in boundary window for training labels. CAM with noise in boundary window for training labels. The first row in each column shows the true labels without any noise and the row below that the prediction done by the network when trained on the noisy example. \emph{Top} to \emph{bottom} activation map: \emph{standing} (\ColorSquare{none}), \emph{begin right step} (\ColorSquare{beginRightStep}), \emph{begin left step} (\ColorSquare{beginLeftStep}), \emph{right step} (\ColorSquare{rightStep}), \emph{left step} (\ColorSquare{leftStep}), \emph{end right step} (\ColorSquare{endRightStep}), \emph{end left step} (\ColorSquare{endLeftStep}), \emph{turn} (\ColorSquare{turnRight}), \emph{reach} (\ColorSquare{reach}) and \emph{retrieve} (\ColorSquare{retrieve})}
\label{fig:cam31}
\end{figure*}

==> sections/06_conclusion.tex <==
\section{Conclusion}
In this paper we introduce the combination of \emph{motion images} and dilated temporal fully-convolutional networks (DT-FCN) for fine-grained semantic frame segmentation of motion capture sequences. We compare three different receptive field size (RFS) versions of our architecture and find that a receptive field of 243 frames, which defines a local structure in our sequences, performs best. This is in contrast to popular claims \cite{bai2018empirical, wavenet} that the RFS has to capture the whole sequence at once.

We analyze the robustness of our model against synthetic noise in the training labels. Our results show that even with 80\% labeling noise, a performance of almost 90\% accuracy in the test set is achieved for the random noise experiment. We compare our model against recent TCN-based baseline models for action segmentation, as well as a popular RNN model and outperform all of them in the experiments. This might be due to the combination of acausal and dilated convolutions in our models, coupled with the fast trainability of TCNs. Our model thus combines both advantages of the presented TCN benchmarks and is over a magnitude faster to train than the LSTM-based method. Additionally, for a more realistic noise experiment, we add noise only in the boundary regions and compare the results to when no information is given in these regions. All models perform better when no information is given. Some of the models, including our's, perform even better when no information is given than when the clean ground truth information is given. This might be due to the inter- and intra-annotator disagreements in the ground truth data, which has been labeled by human ``experts".

%TODO: Write somthing brilliant regarding the interesting finding described in table 7

%During our experiments, we found that simple frame-by-frame test accuracy is an insufficient evaluation criterion for motion segmentation. Over-segmented results can generate a high test accuracy while the generated segments are not useful for subsequent motion modeling techniques. For future work, we propose to develop a novel taking over-segmentation into account. 

There are multiple interesting directions for further research. 
Additional experiments to model inter- and intra-annotator disagreements better should be conducted to better prove the robustness against human error as well as the recording quality of the motion capturing solution. Furthermore, we found that per-frame accuracy does not necessarily capture time-continuities well, we therefore want to explore action detection-based metrics, such as mean  Average Precision with midpoint hit criterion (mAP@mid) \cite{rohrbach2016recognizing, singh2016multi} or mAP with  a  intersection  over  union  (IoU)  overlap  criterion (mAP@k) \cite{richard2016temporal}.  

Finally, although this approach does require considerably less human effort than manual segmentation, further research in semi- and un-supervised learning has to be conducted to make the model more automatic. In this direction domain transfer \cite{ganin2014unsupervised} and few-shot learning \cite{fei2006one} can provide even less human effort. Nevertheless, we believe that our method provides a fruitful tool for motion capture segmentation.
